Are Large Language Models a Good Replacement of Taxonomies?

Large language models (LLMs) demonstrate an impressive ability to internalize knowledge and answer natural language questions. Although previous studies validate that LLMs perform well on general knowledge while presenting poor performance on long-tail nuanced knowledge, the community is still doubtful about whether the traditional knowledge graphs should be replaced by LLMs. In this paper, we ask if the schema of knowledge graph (i.e., taxonomy) is made obsolete by LLMs. Intuitively, LLMs should perform well on common taxonomies and at taxonomy levels that are common to people. Unfortunately, there lacks a comprehensive benchmark that evaluates the LLMs over a wide range of taxonomies from common to specialized domains and at levels from root to leaf so that we can draw a confident conclusion. To narrow the research gap, we constructed a novel taxonomy hierarchical structure discovery benchmark named TaxoGlimpse to evaluate the performance of LLMs over taxonomies. TaxoGlimpse covers ten representative taxonomies from common to specialized domains with in-depth experiments of different levels of entities in this taxonomy from root to leaf. Our comprehensive experiments of eighteen state-of-the-art LLMs under three prompting settings validate that LLMs can still not well capture the knowledge of specialized taxonomies and leaf-level entities.

==> response/general.tex <==
%!TEX root = ../main.tex
\nobalance
\subsection*{Responses to Reviewer Comments}

We appreciate all reviewers for their careful reviews and insightful comments. Based on the comments, we have significantly improved the paper. The revised parts are highlighted in \add{blue} in the paper. 

Our major changes are summarized as follows:

\stitle{New Experiments:}
We have introduced new content and conducted additional experiments to systematically evaluate the performance of LLMs on taxonomy reasoning:

\bi
	\item [{\bf (M1) Four new taxonomies:}] We have added the following new taxonomies in Figure~\ref{fig:example} (Section~\ref{sec:introduction}), Table~\ref{tab:taxonomies} (Section~\ref{sec:benchmark}), and all corresponding experiments (Sections~\ref{sec:settings} and \ref{sec:experiment-results}):

	\bi
		\item eBay (Shopping domain)~\cite{ebay} 
		\item OAE (Medical domain)~\cite{he2014oae} 
		\item Schema.org (General domain)~\cite{guha2016schema} 
		\item GeoNames (Geography domain)~\cite{geonames}
	\ei

	\item [{\bf (M2) Six new baselines:}]
	We have added new baselines (see Section~\ref{sec:llms} {\bf Large Language Models}):

	\bi
		\item Llama-3 8B and 70B~\cite{llama3modelcard}
		\item Mistral-7B-Instruct and Mistral-8*7B-Instruct~\cite{jiang2023mistral,jiang2024mixtral}
		\item Claude-3~\cite{Claude-v3-documentation}
		\item LLMs4OL~\cite{babaei2023llms4ol}
	\ei
	
	where Llama-3s, Mistrals, and Claude-3 are recently released general-purpose LLMs, and LLMs4OL is the state-of-the-art approach that utilizes instruction tuning~\cite{chung2024scaling} based on the Flan-T5-3B model to perform ontology learning tasks.

	\item [{\bf (M3) A new question template:}]	
	We have developed a new question template for multiple-choice questions (MCQs) in Section~\ref{sec:question-design}. Please refer to Table~\ref{tab:question-mcq} for more details.

%	{\color{red} (Discussed in Section~\ref{sec:question-design}, Details presented in Tables~\ref{tab:question}, and~\ref{tab:question-mcq} of our technical report~\cite{technical-report}) } for each taxonomy, two question templates in total.

	\item [{\bf (M4) Three paraphrasing variants:}]	 
	In total, we have devised two question templates (Tables~\ref{tab:question} and \ref{tab:question-mcq}) for each taxonomy.
	Additionally, we conducted experiments using three variations of paraphrasing templates. 
	Due to limitations in space, we present the results in Tables~\ref{tab:exp-main-easy-revision},~\ref{tab:exp-main-hard-revision}, and~\ref{tab:exp-main-mcq-revision} of the response letter, as well as in the GitHub Repository~\cite{taxo-exp}.

%	for each question template, {\color{red} we conducted experiments on three paraphrasing template variants. Results can be found in Tables~\ref{tab:exp-main-easy-revision},~\ref{tab:exp-main-hard-revision}, and~\ref{tab:exp-main-mcq-revision} of the response letter and the Github Repository~\cite{taxo-exp}. }
\ei


\stitle{New Case Study and Discussion:}
We have revised and added the following discussions in Section~\ref{sec:discussion}:


\bi
	\item [{\bf (M5) Limitations of LLMs:}] 
	We elaborated on the limitations of LLMs in addressing specific taxonomies (Section~\ref{sec:limitations}). 
	
	\item [{\bf (M6) A new case study:}] 
	We presented a more comprehensive case study demonstrating the successful integration of LLMs with taxonomies (Section~\ref{sec:discussion-case}).

	\item [{\bf (M7) Scalability:}] 
	We have included a discussion on the scalability of LLMs (Section~\ref{sec:scalability}).
\ei

% \begin{itemize}
%     \item {\bf S1:} We conducted extensive experiments by including {\bf 4 new taxonomies and 6 new baselines}, in total, we have {\bf 10 taxonomies and 18 baselines}. For each taxonomy, we conducted experiments on {\bf 2 different question templates} (True/False and MCQ), each with {\bf 3 paraphrasing variants} to validate the results.
%     \item {\bf S2:} We expanded on the limitations of LLMs in handling specific taxonomies and proposed potential solutions and research directions. Besides, we also provided a discussion on the scalability issue of the LLMs.
%     \item {\bf S3:} We provided more detailed case studies of LLMs successfully integrating with taxonomies, which opens up new research opportunities for the community to work on.
%         \item {\bf S4:} We improved the presentation of figures and paragraphs according to the reviews' suggestions.        
%     \item {\bf S5:} We clarified the claims and aspects by providing additional discussion and explanation in the revised paper.
% \end{itemize}

	% \textbf{\emph{Notations}}: ``R'' is short for reviewer and ``MR'' denotes Meta-Reviewer. ``G'' means general comments, ``W'' represents the weak point, ``V'' means required changes marked by the reviewers, and ``D'' stands for the detailed comment. For example, ``R1-D1'' means the first detailed comments from Reviewer 1.\newline

==> response/meta.tex <==
%!TEX root = ../main.tex
\subsection*{Responses to Meta-Reviewer}

\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D1:} Include a comparison with state-of-the-art taxonomy methods, including more domains of taxonomies.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} We have incorporated a SOTA taxonomy method called LLMs4OL~\cite{babaei2023llms4ol} {\color{black}following the suggestions given by the meta-reviewer in the follow-up email communications and \textbf{R3-D10}} (see {\bf M2}) and introduced four new taxonomies (see {\bf M1}). {\color{red}In general, LLMs4OL boosts the performance of its backbone model Flan-T5-3B by $12.9\%$, $12.9\%$, and $17.0\%$ on the easy, hard, and MCQ datasets, which showcases the significant benefit of performing domain-specific instruction fine-tuning. The inclusion of more domains of taxonomies significantly improves the coverage of our paper and strengthens the key observations.}


\vspace*{1.5ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D2:} Expand on the limitations of LLMs in handling specific taxonomies and propose potential solutions.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]}
We have expanded our discussion on the limitations of LLMs in managing specific taxonomies (see {\bf M5}) and their scalability issues (see {\bf M7}). 
%We have also proposed potential solutions and research directions (\nan{where?}). {\color{black} maybe we remove this line, we only claim in Section~\ref{sec:limitations} that XXX is a promising direction to work on.}

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D3:} Provide more detailed case studies or examples of LLMs successfully integrating with traditional taxonomies.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]}
We have added a new case study (see {\bf M6}). {\color{red}Specifically, our integrated solution saved $59\%$ of the taxonomy maintenance and construction costs, while maintaining precision and recall of over $70\%$ on Amazon Product Category.}


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D4:} Improve Figures 6 and 7.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]}
We have improved Figures 6 and 7 in the previous submission by merging them into a new Figure~\ref{fig:radar} in the revised manuscript.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D5:} Use more diverse benchmarks and baselines.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]}
We have added taxonomies (see {\bf M1}) and baselines (see {\bf M2}). {\color{red}The overall experimental results match our previous observation that, despite some fluctuations and exceptions, the performance of LLMs in general downgrades from common to specialized taxonomies and from root to leaf levels of the taxonomies.}


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D6:} Clarify some of the claims and aspects.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]}
We have addressed all our ambiguous claims raised by the reviewers. 
Please refer to our responses below for each comment.


% \begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable]
% 	\textbf{MR-G:} Thank you for your submission. Following their individual reviews, the reviewers had a discussion of the paper and agreed that the paper should be recommended for revision. While the reviewers urged the authors to look at all of their comments, the following were the points that came up during the discussion that the reviewers really wanted the authors to concentrate on:
	
% 	\textbf{MR-D1:} Include a comparison with state-of-the-art taxonomy methods, including more domains of taxonomies.
    
%     \textbf{MR-D2:} Expand on the limitations of LLMs in handling specific taxonomies and propose potential solutions.
    
%     \textbf{MR-D3:} Provide more detailed case studies or examples of LLMs successfully integrating with traditional taxonomies.
    
%     \textbf{MR-D4:} Improve Figures 6 and 7.
    
%     \textbf{MR-D5:} Use more diverse benchmarks and baselines.

%     \textbf{MR-D6:} Clarify some of the claims and aspects.
% \end{tcolorbox}

%	\textbf{Response to MR-G.} Thanks for your detailed consideration of our approach. We have addressed your comments and revised our paper significantly. In the following part, we will illustrate our revision actions in detail with respect to each of your comments.
	
%	\textbf{Response to MR-D1.} Thank you for your comments. We included a state-of-the-art taxonomy method LLMs4OL and responded to \textbf{R1-V1}, \textbf{R1-W1}, \textbf{R1-D2}, and \textbf{R3-D10}. We included more domains of taxonomies: eBay~\cite{ebay} (Shopping), OAE~\cite{he2014oae} (Medical), Schema.org~\cite{guha2016schema} (General), and GeoNames~\cite{geonames} (Geography) and replied to \textbf{R2-W1}, \textbf{R2-D2}, \textbf{R3-D2}, \textbf{R3-V2}, \textbf{R3-W1}, \textbf{R3-D3}, and \textbf{R3-V3} (Changes summarized in {\bf S1}).
	
%	\textbf{Response to MR-D2.} Thank you for your comments. We have improved the discussion on the limitations of LLMs and proposed potential solutions. Please check the response to \textbf{R1-V1}, \textbf{R1-W2}, \textbf{R1-W3}, and \textbf{R1-D4} (Changes summarized in {\bf S2}).
	
	% \textbf{Response to MR-D3.} Thanks for your comments. We included a case study of the integration of LLMs with traditional taxonomies and replied to \textbf{R1-V3} and \textbf{R1-D3} (Changes summarized in {\bf S3}).
	
	% \textbf{Response to MR-D4.} We appreciate your comments. We have improved the visualizations of Figures 6 and 7. Please refer to response to \textbf{R2-V2}, \textbf{R2-W3}, and \textbf{R2-D3} for details (Changes summarized in {\bf S4}).
	
	% \textbf{Response to MR-D5.} Thank you. We included more diverse benchmarks and baselines in our experiments. Please check the reply to \textbf{R3-V3}, \textbf{R3-W2}, \textbf{R3-D7}, and \textbf{R3-D10} for details (Changes summarized in {\bf S1}).

    %     \textbf{Response to MR-D6.} Thanks for your comments. We clarify the details by responding to \textbf{R3-V1}, \textbf{R3-W3}, \textbf{R3-D2}, \textbf{R3-D4}, \textbf{R3-D5}, \textbf{R3-D6}, \textbf{R3-D8}, and \textbf{R3-D9} (Changes summarized in {\bf S5}).
	

==> response/response1.tex <==
%!TEX root = ../main.tex	
\subsection*{Responses to Reviewer 1}

\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 1:} Include a comparison with state-of-the-art taxonomy methods.

    \textbf{W1:} The experimental setup lacks comparison with state-of-the-art taxonomy approaches.

    \textbf{D2:} The paper lacks a direct comparison with the latest taxonomy approaches, which could have strengthened the argument for LLMs as a viable alternative.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} 
We have incorporated LLMs4OL~\cite{babaei2023llms4ol} as the SOTA taxonomy method (see {\bf M2}). {\color{black}The selection of LLMs4OL follows the suggestions given by the meta-reviewer in the follow-up email communications and \textbf{R3-D10}. The reason why we did not include taxonomy construction approaches in comparison is those approaches mainly utilize textual corpus as knowledge sources, extract the entities and relations, and then construct the taxonomy, which is not comparable in our settings, due to the absence of accompanying textual corpus for the taxonomies we collected~\cite{asim2018survey, babaei2023llms4ol, lourdusamy2020survey}. As suggested by \textbf{R3-D10}, LLMs4OL is the only nearest system and indeed the only comparable taxonomy method under our settings so we only include this SOTA method in the experiments. {\color{red}In general, LLMs4OL boosts the performance of its backbone model Flan-T5-3B by $12.9\%$, $12.9\%$, and $17.0\%$ on the easy, hard, and MCQ datasets, which showcases the significant benefit of performing domain-specific instruction fine-tuning.}}

%\textbf{Response to R1-V1, R1-W1, and R1-D2.} Thank you for your comments. We agree that including a comparison with the state-of-the-art taxonomy methods should be helpful for our manuscript. Considering that the task of our paper is to study whether LLMs have internalized taxonomy knowledge, we followed the suggestion by \textbf{R3-D10} and included LLMs4OL~\cite{babaei2023llms4ol} as the state-of-the-art taxonomy method. LLMs4OL is the state-of-the-art approach that utilizes instruction tuning~\cite{chung2024scaling} based on the Flan-T5-3B model to perform ontology learning tasks. We did not compare with the taxonomy construction approaches since those approaches mainly utilize textual corpus as knowledge sources, extract the entities and relations, and then construct the taxonomy, which is not comparable in our settings, since there is no accompanying textual corpus for the taxonomies we collected. The inclusion of LLMs4OL provides valuable insight for overcoming the limitations of LLMs, which strengthens the argument for LLMs as a viable alternative. Please see Section~\ref{sec:llms} of the revised manuscript for a detailed description of LLMs4OL.

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 2:} Expand on the limitations of LLMs in handling specific taxonomies and propose potential solutions.

\textbf{W2:} There is an insufficient discussion on the impact of LLM limitations on taxonomy replacement.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} 
We have revised Section~\ref{sec:limitations} to provide a more detailed explanation of the limitations of LLMs (see {\bf M5}). A key limitation stems from the domain specificity of LLMs. Without domain-specific instruction fine-tuning, LLMs often exhibit poor performance in the lower levels of specialized taxonomies, hindering their ability to replace taxonomy structures. One potential solution is to substitute taxonomy structures at levels where LLMs can consistently achieve high performance, as shown in the new case study (see {\bf M6}).

Moreover, our experiments indicate that domain-specific instruction fine-tuning may {\color{black}enhance the performance of LLMs on taxonomies.} Although this approach necessitates high-quality labeled data and incurs substantial training costs, we are optimistic that these challenges can be mitigated through domain adaptation techniques~\cite{kocielnik2023can, fang2024source,han2024chatgpt}, which presents a promising avenue for future research.


%Thank you for your valuable comments. We agree that the limitation of LLM replacement of taxonomy is not discussed thoroughly. We thus provide a more in-depth discussion in Section~\ref{sec:limitations} of the revised manuscript. Specifically, a major limitation lies in the domain specificity of the LLMs. Without introducing domain-specific instruction fine-tuning, the LLMs tend to perform poorly near the low levels of the specialized taxonomies, which is a limitation for adopting LLMs to replace the taxonomy structures. One possible solution is to replace the taxonomy structures at levels where the LLMs can achieve high and stable performance. We also provided an example of taxonomy structure replacement in Section~\ref{sec:discussion-case} and \textbf{Response to R1-V3, and R1-D3} on this solution. Besides, our experiments show that domain-specific instruction fine-tuning could be a potential solution to boost the performance of LLMs at the low levels of the specialized taxonomies. Despite the fact that domain-specific instruction fine-tuning requires high-quality labeled data and induces high training costs, we believe these issues could be resolved by introducing domain adaptation techniques as discussed by some pilot works~\cite{kocielnik2023can, fang2024source,han2024chatgpt}. However, the effectiveness of these techniques on taxonomies is not yet validated and we believe this should be a promising future direction for the community to explore.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 3:} Provide more detailed case studies or examples of LLMs successfully integrating with traditional taxonomies.

\textbf{D3:} The discussion on integrating LLMs with traditional taxonomies is insightful, yet more concrete examples or case studies would enhance its applicability.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} 
We have incorporated a comprehensive case study illustrating the successful integration of LLMs with conventional taxonomies (see {\bf M6}). Our study demonstrates that by substituting level 4 or lower concepts of the Amazon Product Category with Llama-2-70B, we can reduce taxonomy construction and maintenance costs by 59\%, while maintaining precision and recall levels above 70\%. Please check Section~\ref{sec:discussion-case} for more details. %For further details, please consult Section~\ref{sec:discussion-case} of the revised manuscript.


%\textbf{Response to R1-V3, and R1-D3.} Thank you for your concrete comments. We have included a detailed case study of LLMs successfully integrating with traditional taxonomies. Specifically, we have shown that by replacing the level 4 or lower concepts of the Amazon Product Category with Llama-2-70B, we can save $59\%$ taxonomy construction and maintenance costs, while achieving precision and recall of over $70\%$. Please refer to Section~\ref{sec:discussion-case} of the revised manuscript for details.   

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{W3:} The paper could benefit from a deeper analysis of domain-specific LLM training for taxonomy tasks.

\textbf{D4:} The experimental design is robust, but the coverage of certain claims, specifically regarding scalability and domain specificity, is insufficient.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} 
For {\bf domain specificity}, we have added a paragraph ``Domain-specific Fine-tuning'' discussing the effect of conducting domain-specific instruction fine-tuning in Section~\ref{sec:exp-normal-methods}. Specifically, we compare the performances of LLMs4OL (see {\bf M2}) and the original Flan-T5-3B model. In the revised manuscript, we provide the comparison as follows: \textit{The averaged accuracy over all taxonomies of LLMs4OL boosts the performance of Flan-T5-3B by $12.9\%$, $12.9\%$, and $17.0\%$ on the easy, hard, and MCQ datasets, which showcases the significant benefit of performing domain-specific instruction fine-tuning.} 

For {\bf scalability}, we have added a new scalability section in Section~\ref{sec:scalability} of the revised manuscript. \textit{We analyze the scalability of the LLM series by recording the GPU RAM and the average time costs induced by each LLM model in the corresponding LLM series during the inference of zero-shot taxonomy questions. The experimental results are presented in Figure~\ref{fig:scalability}. Specifically, we considered the scalability of six open-sourced LLM series: Llama-2s, Llama-3s, Vicunas, Flan-T5s, Falcons, and Mistrals. We observe that Flan-T5s, Vicunas, and Llama-3s present relatively good scalability, as the model size grows, the inference time does not increase significantly, which is especially important for their adoption in real-world taxonomy-related applications.}

  %  \textbf{Response to R1-V2, and R1-W2.} Thank you for your valuable comments. We agree that the limitation of LLM replacement of taxonomy is not discussed thoroughly. We thus provide a more in-depth discussion in Section~\ref{sec:limitations} of the revised manuscript. Specifically, a major limitation lies in the domain specificity of the LLMs. Without introducing domain-specific instruction fine-tuning, the LLMs tend to perform poorly near the low levels of the specialized taxonomies, which is a limitation for adopting LLMs to replace the taxonomy structures. One possible solution is to replace the taxonomy structures at levels where the LLMs can achieve high and stable performance. We also provided an example of taxonomy structure replacement in Section~\ref{sec:discussion-case} and \textbf{Response to R1-V3, and R1-D3} on this solution. Besides, our experiments show that domain-specific instruction fine-tuning could be a potential solution to boost the performance of LLMs at the low levels of the specialized taxonomies. Despite the fact that domain-specific instruction fine-tuning requires high-quality labeled data and induces high training costs, we believe these issues could be resolved by introducing domain adaptation techniques as discussed by some pilot works~\cite{kocielnik2023can, fang2024source,han2024chatgpt}. However, the effectiveness of these techniques on taxonomies is not yet validated and we believe this should be a promising future direction for the community to explore.

    % \textbf{Response to R1-W3, and R1-D4.} Thanks for your valuable comments. We agree that providing more discussion on domain specificity and scalability would improve the value of our manuscript. We added a paragraph \textbf{Domain-specific Fine-tuning.} discussing the effect of conducting domain-specific instruction fine-tuning in Section~\ref{sec:exp-normal-methods}. Specifically, we compare the performances of LLMs4OL (which is the Flan-T5-3B we adapted to each taxonomy with instruction fine-tuning guidance discussed in their paper~\cite{babaei2023llms4ol}) and the original Flan-T5-3B model. In the revised manuscript, we provide the comparison as follows: \textit{The averaged accuracy over all taxonomies of LLMs4OL boosts the performance of Flan-T5-3B for $12.9\%$, $12.9\%$, and $17.0\%$ on the easy, hard, and MCQ datasets, which showcases the significant benefit of performing domain-specific instruction fine-tuning.} We believe that by discussing the effect of introducing domain-specific instruction fine-tuning, we provide the audience with a better understanding of the benefit of domain-specific LLM training (domain specificity). Hopefully, your concerns about domain specificity can be resolved. 
    
    % We added an additional scalability section in Section~\ref{sec:scalability} of the revised manuscript: \textit{We analyze the scalability of the LLM series by recording the GPU RAM and the average time costs induced by each LLM model in the corresponding LLM series during the inference of zero-shot taxonomy questions. The experimental results are presented in Figure~\ref{fig:scalability}. Specifically, we considered the scalability of six open-sourced LLM series: Llama-2s, Llama-3s, Vicunas, Flan-T5s, Falcons, and Mistrals. We observe that Flan-T5s, Vicunas, and Llama-3s present relatively good scalability since as the model size grows, the inference time does not increase significantly, which is especially important for their adoption in real-world taxonomy-related applications.}

\begin{comment}
    \begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{./img/scalability.pdf}
  \caption{The Scalability of Different Model Series.}
  \label{fig:scalability}
\end{figure}
\end{comment}
    
    
  

==> response/response2.tex <==
%!TEX root = ../main.tex	
\subsection*{Responses to Reviewer 2}

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 1:} Addressing D2.

\textbf{W1:} Covering a limited number of taxonomies in the benchmark.

\textbf{D2:} Although explicitly stated by the authors, the paper covers a limited number of taxonomies. I believe the paper should have included many more taxonomies from different domains as it is the first attempt to build and introduce the proposed benchmark to the community. I believe the authors could find many more taxonomies from different fields in the Semantic Web literature. For example, the linked open data cloud (http://cas.lod-cloud.net/) has thousands of knowledge graphs, many of which include taxonomies of the entities they cover.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} We followed your suggestions to search for more taxonomies from the linked open data cloud and found the GeoNames taxonomy~\cite{geonames} (Geography domain) and the OAE taxonomy~\cite{he2014oae, OAE} (Medical domain) (see {\bf M1}). Specifically, the GeoNames taxonomy is representative of the geography domain covering a two-level classification of the common geographical concepts. The OAE (Ontology of Adverse Events) taxonomy is a taxonomy specialized for adverse events in the medical domain. 

We further included the Schema.org taxonomy~\cite{guha2016schema} (General domain) and the eBay taxonomy~\cite{ebay} (Shopping domain) to enrich the range of coverage of our benchmark (see {\bf M1}). The Schema.org taxonomy is a general domain taxonomy covering a wide range of concepts on the internet and serves as the basis for other general-purpose knowledge bases such as YAGO~\cite{suchanek2007yago}.

Please see Section~\ref{sec:data-collection} for the details of these new taxonomies. {\color{red}In general, the experimental results on the newly added taxonomies match our previous key observations of LLMs' performance on the common-to-specialized domains and the root-to-leaf levels.}

%\textbf{Response to R2-V1, R2-W1, and R2-D2.} Thank you for your helpful comments. We agree that our manuscript can greatly benefit from including more taxonomies in the benchmark. Therefore, we followed your suggestions to search for more taxonomies from the linked open data cloud and found the GeoNames taxonomy~\cite{geonames} (Geography domain) and the OAE taxonomy~\cite{he2014oae, OAE} (Medical domain). Specifically, the GeoNames taxonomy is representative of the geography domain covering a two-level classification of the common geographical concepts. The OAE (Ontology of Adverse Events) taxonomy is a taxonomy specialized for adverse events in the medical domain. The OAE taxonomy has been developed to standardize the annotation of adverse events, integrate various adverse event data, and support computer-assisted reasoning. We further included the Schema.org taxonomy~\cite{guha2016schema} (General domain) and the eBay taxonomy~\cite{ebay} (Shopping domain) to enrich the range of coverage of our benchmark. The Schema.org taxonomy is a general domain taxonomy covering a wide range of concepts on the internet and serves as the basis for other general-purpose knowledge bases such as YAGO~\cite{suchanek2007yago}. The eBay taxonomy is from ebay.com, which is a popular online shopping platform. Please refer to Section~\ref{sec:data-collection} for the details of these newly added taxonomies.
 
\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 2:} Addressing D3.

\textbf{W3:} Some visualizations need improvements.

\textbf{D3:} Figures 6 and 7 are not visually appealing. You need to find a point in Figure 6(a), then move to compare to its corresponding point in Figures 6(b) and 6(c) to make a sense of the comparison. These charts are supposed to be used to differentiate between two scenarios on the same chart (e.g., zero-shot vs. few-shot in the same chart). Therefore, maybe a smaller subset of the LLMs (that differ significantly among the prompting settings) could have been included, where each figure shows only the three prompting settings for one selected LLM. And then, we could have several of these figures for the subset of the LLMs chosen.
\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} Thank you for your valuable feedback. Based on your suggestion, we have merged Figures~6 and 7 in the previous submission into Figure~\ref{fig:radar} in the revised manuscript. 
%
Specifically, Figure~\ref{fig:radar} now presents the accuracy results for  GPT-4, Flan-T5-11B, and Llama-2-7B models, along with the miss rate result for the Llama-2-7B model. By following the analysis we presented in Section~\ref{sec:exp-prompting}, we hope the audience can gain a deeper understanding of our findings regarding different prompting settings.


%\textbf{Response to R2-V2, R2-W3, and R2-D3.} Thank you for your helpful comments. We agree that the visualizations of Figures 6 and 7 in the original manuscript need improvements. We thus updated the visualizations for the few-shot and CoT experiments by only presenting the essential LLMs that are mentioned in our analysis of the results. We present the zero-shot, few-shot, and CoT results for each selected LLM in one figure so that the audience does not need to align different lines in different charts together to get a clear understanding of the experimental results. Specifically, we presented the accuracy results for GPT-4, Flan-T5-11B, and Llama-2-7B models, and the miss rate result for the Llama-2-7B model in Figure~\ref{fig:radar} of our revised manuscript. The reason why we selected GPT-4 and Flan-T5-11B is that these two are the representative close-sourced and open-sourced LLMs that we observed some valuable insights respectively. Besides, we also selected Llama-2-7B, which presents significant changes in its performance among different prompting settings. We believe in this way the audience can have a better understanding of the few-shot and CoT results. By following the analysis we presented in Section~\ref{sec:exp-prompting}, we hope the audience can gain a deeper understanding of our findings regarding different prompting settings. Please check the updated figures in Figure~\ref{fig:radar} of the revised paper.  

\begin{comment}

 \begin{figure*}[htbp]
\centering
  \subfigure[GPT-4, accuracy]{
\label{subfig:radar-gpt4-acc}
  \includegraphics[width=0.235\linewidth]{./img/exp-figures/gpt-4-acc.pdf}}
  \subfigure[Flan-T5-11B, accuracy]{
\label{subfig:radar-flan-t5-acc}
  \includegraphics[width=0.235\linewidth]{./img/exp-figures/flan-t5-11b-acc.pdf}}
  \subfigure[Llama-2-7B, accuracy]{
\label{subfig:radar-llama-acc}
  \includegraphics[width=0.235\linewidth]{./img/exp-figures/llama-2-7b-acc.pdf}}
  \subfigure[Llama-2-7B, miss rate]{
\label{subfig:radar-llama-miss}
  \includegraphics[width=0.235\linewidth]{./img/exp-figures/llama-2-7b-miss.pdf}}
  \vspace{-1em}
  \caption{Radar charts for representative LLMs under different prompting settings in hard datasets.}
  \label{fig:radar-response}
  \vspace{-1em}
\end{figure*}
   
\end{comment}

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{W2:} Limited number of new insights.

\textbf{D1:} Several of the shared findings were discussed before in the literature or could be considered common-sense knowledge in the field. It is known that LLMs's knowledge is limited in covering long-tail entities. This includes less-known and less-covered taxonomies in training data. Therefore, these findings cannot be considered as one of the contributions of this paper.

\end{tcolorbox}

\vspace*{-2ex}
\stitle{[A]} We agree with the reviewer that some of the insights seem to be common-sense knowledge. By extending the coverage of domains and LLMs in our experiments (Sections~\ref{sec:settings} and \ref{sec:experiment-results}) and discussion (Section~\ref{sec:discussion}), we update, refine, and summarize our insights as follows:

\sstab
(1) We have observed that LLMs perform well on common taxonomies but exhibit instability and lower performance on specialized taxonomies in Section~\ref{sec:exp-common-to-specialized}. While these findings align with the general understanding in the community that LLMs struggle with long-tailed knowledge, {\em previous studies have not explicitly defined taxonomies into common and specialized categories or validated this hypothesis using taxonomic data}.
	
\sstab
(2) We have observed a root-to-leaf phenomenon in the behavior of LLMs across most taxonomies and investigated the reasons for exceptional cases in Section~\ref{sec:exp-root-to-leaf}. Unlike entities in standard knowledge bases, the popularity of entities at different levels of taxonomy is not clearly delineated. For instance, in domains like Biology, one might intuitively expect lower-level concepts such as ``Cat'' and ``Dog'' to be more popular than higher-level concepts like ``Carnivores''. Consequently, {\em the root-to-leaf phenomenon is not always as straightforward as it may seem}.

\sstab
(3) We have validated several conventional methods to enhance LLM performance and discovered that {\em larger model sizes and domain-agnostic fine-tuning do not consistently improve LLM performance on taxonomy tasks} in Section~\ref{sec:exp-normal-methods}. This aspect has not been extensively explored within the community.

\sstab
(4) 
We have evaluated the performance of various prompting settings that are claimed to be beneficial in Section~\ref{sec:exp-prompting}. Our findings indicate that {\em few-shot prompting has a positive effect in reducing miss rates, whereas CoT prompting negatively impacts the performance of LLMs on taxonomy tasks}.

\sstab
(5) We have updated the instance typing experiments, which validate the performance of LLMs in performing instance typing to the parent, grandparent, ..., root in Section~\ref{sec:exp-instance}. This section {\em validates the stability of LLMs and is of great value in the real-world replacement of taxonomy}. 

\sstab
(6) We have included a new scalability analysis in Section~\ref{sec:scalability} (see {\bf M7}) of different model series, which {\em gives concrete advice for the audience to select LLMs for their actual usage}. 

\sstab
(7) We provided a real case study in Section~\ref{sec:discussion-case} (see {\bf M6}) of LLM integrating with taxonomy, which {\em gives a concrete example for the future vision of LLMs and taxonomy} we suggested in Section~\ref{sec:dicussion-future}.

{\color{red}In summary, we are the first work to comprehensively study the performance of LLMs on taxonomies from common to specialized domains with a detailed granularity from root to leaf levels. Several important hypotheses are verified on taxonomic data for the first time. During the validation of the hypotheses, we identify some interesting observations that are not completely straightforward or are discrepant from the prior common sense in other application areas. These interesting insights can indeed spark innovation in the future development of ontology learning.}
%\ei

% \textbf{Response to R2-W2, and R2-D1.} Thank you for your comments. We agree that some of the insights presented were similar to the findings discussed before. By extending the coverage of domains and LLMs in our experiments we update, refine, and summarize our insights as follows: 1) We observe that the LLMs perform well on common taxonomies while becoming unstable and less satisfactory on specialized taxonomies. Although the findings match with the common sense of the community that the LLMs are limited in covering long-tailed knowledge, no previous study actually clearly defines the taxonomies into common and specialized and thereafter validates this hypothesis on taxonomic data. 2) We find that the LLMs tend to present a root-to-leaf phenomenon on most taxonomies and examine the reasons for exceptional cases. Different from entities in normal knowledge bases, the popularity of the entities in different levels of taxonomy is not clearly defined. In some domains such as Biology, intuitively, the lower level concepts such as Cat and Dog should be more popular in comparison with the higher level concepts such as Carnivals. Therefore, the root-to-leaf phenomenon is indeed not as obvious as we intuitively think it is. 3) We validate several normal methods that claim to improve the performance of LLMs and it turns out that larger model sizes and domain-agnostic fine-tuning cannot stably improve the performance of LLMs on taxonomy tasks, which is indeed unexplored by the community. The domain-specific fine-tuning we added as suggested by \textbf{R1-W3} is shown to be beneficial and can be applied to strengthen the performance of LLMs in real-world applications. 4) We validate the performance of applying different prompting settings that claim to be beneficial. It turns out that few-shot prompting has a positive effect in reducing the miss rates, while CoT prompting brings a negative influence on the performance of the LLMs on taxonomy tasks. 5) We update the instance typing experiments, which validate the performance of LLMs in performing instance typing to the parent, grandparent, ..., root. This section validates the stability of LLMs and is of great value in the real-world replacement of taxonomy. 6) As suggested by \textbf{R1-D4}, we included scalability analysis of different model series, which gives concrete advice for the audience to select LLMs for their actual usage. 7) We provided a real case study of LLM integrating with taxonomy, as suggested by \textbf{R1-D3}, which gives a concrete example for the future vision of LLMs and taxonomy we suggested in Section~\ref{sec:dicussion-future}. The discussion and analysis of the results provide future research directions for the community to work on. 


==> response/response3.tex <==
%!TEX root = ../main.tex	
\subsection*{Responses to Reviewer 3}

\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{Required Revision 1:} Further clarifications with respect to some claims/aspects. (D2, D4, D5, D6, D8, D9)

\textbf{Required Revision 2:} The experiments need to include more domains of taxonomies. (D2, D3) 

\textbf{Required Revision 3:} Use of diverse benchmarks and baselines. (D7, D10)

\textbf{W1:} The construction of the benchmark is not very convincing.

\textbf{W2:} The experiments are not thorough enough for a EA\&B paper.

\textbf{W3:} Some of the details are skipped. Please refer detailed feedback.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]} Please refer to our responses to your comments D1--D10 below.

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D1:} It is commendable that the paper has provided its code and used publicly available datasets.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
Thanks for your comments. We have made our code and datasets publicly available on GitHub (\url{https://github.com/ysunbp/TaxoGlimpse}).

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D2:} Section 1: the definition of "common" vs "specialized" is only vaguely explained. For example, one may argue that "Home \& Garden" is indeed a specialized domain as compared to "People". How about using more general purpose taxonomy as those of Wikidata or Schema.org (used by YAGO for e.g.)?
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
{\color{red}Thank you for your insightful comments. We agree that including the general-purpose taxonomy can improve the coverage of the paper. We therefore followed your suggestions and included Schema.org into our benchmark (see {\bf M1}). We acknowledge that formally distinguishing between common and specialized taxonomies is a complex task without universal definitions. Instead, {\bf our focus} is to offer a rough, relative ranking of the commonness of different taxonomies, which aligns with the common understanding and allows us to summarize the interesting observations that spark the innovation of the ontology learning field.
}

\stitle{New measure of popularity.} In our revised manuscript (Figure~\ref{fig:popularity} at Section~\ref{sec:benchmark}), we classify taxonomies that cover commonly known and accessible entities as `common taxonomies', and those that are domain-specific and likely accessed by experts as `specialized taxonomies'. We categorized the ten taxonomies into these types based on the average number of Google search exact match results returned for 100 randomly sampled concepts from each taxonomy. This approach provides a rough indication of the taxonomies' commonness: a taxonomy with abundant search results likely contains widely accessible information, while a taxonomy with scarce search results is likely specialized and used by domain experts. Similar methods have been previously used to estimate content popularity~\cite{malagon2023measuring, genoe2021applying}.

We recognize that even common taxonomies may include somewhat domain-specific knowledge, \eg your Home \& Garden and People example. Our classification method above allows us to compare the overall commonness of different taxonomies, providing a rough ranking from common to specialized taxonomies for ease of discussion and demonstration.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D3:} Figure 2: There is a sudden fall in popularity after Amazon. There is a need for a better medium popularity dataset.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
Thanks for your comments. For a more diverse and comprehensive evaluation, we have added four new taxonomies (see {\bf M1}).

Moreover, our previous measure of popularity based on the number of search results by searching the taxonomy names may not accurately reflect the popularity of the content of the taxonomy. {\color{black} Our original measure of popularity directly records the number of Google search results returned by searching the names of the taxonomies. In our previous popularity figure, Google and Amazon shopping taxonomies have significantly more search results returned than the rest of the taxonomies (sudden fall in popularity after Amazon). After careful analysis, we believe the reason why Google and Amazon shopping taxonomies have significantly more results is that the words `Google' and `Amazon' are very popular words on the internet, which bias the search results of their corresponding taxonomy names `Google Product Category' and `Amazon Product Category' by including many similar yet irrelevant results. As a result, a sudden fall in popularity after Amazon occurs in our previous popularity figure. }

{\color{black}Besides, we discover that using the names of the taxonomies as the indicator for popularity would not reflect the popularity of their content perfectly.} Based on your suggestion in {\bf D2}, we have updated our approach to measuring popularity. Instead of focusing on the popularity of taxonomy names, we now measure the popularity of individual taxonomy concepts. This change has resulted in a more reasonable measurement of popularity, resolving the issue of sudden drops in popularity. Please refer to Figure~\ref{fig:popularity} for the updated popularity figure.

%\textbf{Response to R3-D3.} Thank you for your comments. Indeed, our previous measure of popularity based on the number of search results by searching the taxonomy names may not accurately reflect the popularity of the content of the taxonomy. Firstly, some taxonomies do not have a formal or universal name, such as eBay categories~\cite{ebay} (do not have a formal name) and Google Product Category~\cite{Google-shopping-tax} (refer to as ``Google Product Category'' on its introductory page~\cite{Google-shopping-intro}, while as ``Google Product Taxonomy'' in its file name~\cite{Google-shopping-tax}). Besides, the names of the taxonomies themselves would bias the results. Many irrelevant results are returned when searching Amazon Product Category and Google Product Category since the words Amazon and Google are common words on the internet. As a result, the estimated popularity of the Amazon Product Category and the Google Product Category is significantly higher than the rest of the taxonomies. Your comment \textbf{R3-D2} (\textit{For example, one may argue that ``Home \& Garden'' is indeed a specialized domain as compared to ``People''.}) enlightens us to think deeper about the popularity measure of the taxonomies. The popularity of taxonomy should be measured by the popularity of the taxonomy concepts (such as ``Home \& Garden'' and ``People'') inside instead of that of taxonomy names. Therefore, we rectified our measure of popularity as follows: we randomly sampled 100 concepts from each taxonomy and then recorded the average number of results returned by Google.com by searching for the concept names. To avoid the irrelevant content returned, we adopted the exact match searching mode of the Google search engine. The updated popularity is shown in Figure~\ref{fig:popularity}. We observe that the sudden fall in popularity problem is resolved after we adopted the rectified measure of popularity. We have updated Figure~\ref{fig:popularity} and the corresponding description in the revised manuscript.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D4:} Section 2.1: The Amazon Product Category was crawled to collect it from BrowseNodes. What is the percentage coverage in this case w.r.t. the original catalog? The site mentions having only popular categories, thus, they could bias the end results.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
The main reason why we cannot obtain the full, original Amazon product taxonomy is that the complete Amazon Product Category is not publicly available, and Amazon only discloses the root categories on its official website (\url{https://www.amazon.com/}).

To address your coverage concern, we compared the root categories of the taxonomy we collected from BrowseNodes with the Amazon root categories. Our collected taxonomy covers 39 out of 55 of the latest root categories of Amazon.com, which represents {\bf over $70\%$ coverage}.

To ensure a comprehensive evaluation of LLMs for the shopping domain taxonomy, we have added a new, {\color{black}complete eBay taxonomy used by eBay.com (\url{https://www.ebay.com/n/all-categories})} (see {\bf M1}) in addition to the previously considered Amazon and Google Product taxonomies. This addition strengthens the reliability of our observations in the shopping domain. We have found that the results across the three shopping taxonomies are consistent and do not significantly influence our observations and insights. For more details, please refer to Section~\ref{sec:data-collection}.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D5:} Table 1: It is unclear how the number of entities is correlated with the specialization of the taxonomy. In general, the features chosen (levels, trees, etc.) to represent the diversity of the taxonomies are not concretely justified. What is the number of questions per taxonomy?
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
We apologize for the confusion. The number of entities in a taxonomy is not necessarily correlated with its specialization. For example, eBay (shopping domain) has 595 entities, while NCBI (Biology domain) has 2,190,125 entities (see Table~\ref{tab:taxonomies}), yet eBay is much more popular than NCBI (see Figure~\ref{fig:popularity}).

According to Wikipedia, a taxonomy is a scheme of classification, especially a hierarchical classification, in which things are organized into groups or types. Therefore, in our study, we chose features that systematically cover the scale of the taxonomies (number of entities), the depth of the taxonomies (number of levels), and the width of the taxonomies (number of trees). {\color{black}By including taxonomies with diverse characteristics (such as scale, depth, and width), we can comprehensively evaluate taxonomies with diverse morphologies. }We have clarified these choices in Section~\ref{sec:data-collection} and updated Table~\ref{tab:taxonomies} accordingly.

Regarding the number of questions per taxonomy, we acknowledge that the original presentation of Table~\ref{tab:data-stat} may not have been clear. To address this, we have added new ``Total'' rows at the bottom of Table~\ref{tab:data-stat} for the total number of questions per taxonomy.

%Indeed the number of entities is not correlated with the specialization of the taxonomy. In Section~\ref{sec:data-collection} of the original manuscript, we stated that ``\textit{Apart from the popularity of taxonomies, we also considered the characteristics of different taxonomies. As shown in Table~\ref{tab:taxonomies}, the selected taxonomies have a range of cover of different numbers of entities (from 2K to 2M), number of levels (from 4 to 7), and number of tree roots (from 13 to 245), represent well the overall distribution of taxonomies in different application scenarios.}'', which means the taxonomies we chose for evaluation are not only diverse in popularity but also have diverse features such as number of entities, number of levels, and number of tree roots. As a result, from the morphological perspective, the selected taxonomies have diverse structures, which means they are representative candidates for our evaluation. 

%The main reason why we presented levels, trees, etc in Table~\ref{tab:taxonomies} is that these features describe the basic information of the taxonomies well. By having these features, the audience can learn about the scale of the taxonomies (number of entities), the depth of the taxonomies (number of levels), the width of the taxonomies (number of trees), the rough shape of the taxonomies (number of nodes and classes in each level), which gives the audience rough ideas of the characteristics of the taxonomies. We have updated Section~\ref{sec:data-collection} to explain further the relationship between the diversity of features and the representative of the taxonomies and justify the selection of these features. Specifically, we modified the paragraph into: ``\textit{Apart from the popularity of taxonomies, we also considered the characteristics of different taxonomies. As shown in Table~\ref{tab:taxonomies}, the characteristics we selected give the audience the basic information about the scale of the taxonomies (number of entities), the depth of the taxonomies (number of levels), the width of the taxonomies (number of trees), the rough shape of the taxonomies (number of nodes and classes in each level). The selected taxonomies have a range of cover of different numbers of entities (from 500 to 2M), number of levels (from 2 to 7), and number of tree roots (from 3 to 245), representing well the diverse distribution of the morphology of taxonomies in different application domains and scenarios.}'' As for the number of questions per taxonomy, we admit that our original presentation of Table~\ref{tab:data-stat} is not clear enough, we therefore added a new row at the bottom of the table recording the total number of questions per taxonomy. Please check Table~\ref{tab:data-stat} in the revised manuscript for details.

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D6:} Section 2.2: ``We observed similar results when using slight paraphrasing of the templates, so will report results on these templates only.'': What is meant by ``slight'' paraphrasing? How similar were the results?
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
We have revised the explanation of the ``slight paraphrasing'' in Section~\ref{sec:question-design}. Next we will explain by examples.

\stitle{True/False Questions.} Take the original template in the health domain as an example, which we denote as template v1: 

\bi
   \item {\bf v1:} Is $<$child-type$>$ \textbf{a type of} $<$parent-type$>$? answer with (Yes/No/I don't know)
\ei

The slight paraphrasing process replaces the words ``a type of'' in the original templates {\color{black}with the synonyms}: ``a kind of'' and ``a sort of'', resulting in two variant templates v2 and v3: 

\bi
   \item {\bf v2:} Is $<$child-type$>$ \textbf{a kind of} $<$parent-type$>$? answer with (Yes/No/I don't know)
   \item {\bf v3:} Is $<$child-type$>$ \textbf{a sort of} $<$parent-type$>$? answer with (Yes/No/I don't know)
\ei

\stitle{MCQ Questions.}
Similarly, for the multiple-choice question (MCQ) template, consider the template:

\bi
   \item {\bf v1:} What is the most \textbf{appropriate} supertype of $<$child-type$>$? A) B) C) D).
\ei

We replace the word ``appropriate'' with ``suitable'' and ``proper'', resulting in two variants templates v2 and v3 as:

\bi
   \item {\bf v2:} What is the most \textbf{suitable} supertype of $<$child-type$>$? A) B) C) D)
   \item {\bf v3:} What is the most \textbf{proper} supertype of $<$child-type$>$? A) B) C) D)
\ei

We present the accuracy and standard deviation for all the LLMs with different template variants on all the Easy, Hard, and MCQ datasets in Tables~\ref{tab:exp-main-easy-revision},~\ref{tab:exp-main-hard-revision}, and~\ref{tab:exp-main-mcq-revision} respectively. We observe that most LLMs have stable performance on all the taxonomies with different template variants. Specifically, we computed the average standard deviation for each LLM on the ten taxonomies. The maximum averaged standard deviations are $0.028$, $0.022$, and $0.019$ for the Easy, Hard, and MCQ datasets respectively. 

Due to space constraints, we will put the above results in our public GitHub repo~\cite{taxo-exp}.

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D7:} With LLMs, it is possible to have varied results on slight changes in the language structure and end task. Thus, simple True/False questions are in no way an exhaustive evaluation for LLMs over taxonomy-based end tasks. The authors cite [21] to suggest that True/False questions are better than MCQs for humans. This is, however, not conclusive for machine-based LLMs.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
We agree that the question templates might influence the evaluation results. Therefore, we included the experiments on MCQs in the revised manuscript. Please check Section~\ref{sec:question-design} of the revised manuscript for details of the question templates and Table~\ref{tab:exp-mcq} in the technical report~\cite{technical-report} for the experimental results. {\color{red}Comparing the experimental results between the Easy, Hard, and MCQ datasets, we observe that providing MCQ options significantly reduces the miss rates of the LLMs. For instance, the average miss rates of the Llama-3-70B model reduce from $0.151$ on the Hard datasets to $0.005$ on the MCQ datasets. The average accuracy of Llama-3-70B in turn rises from $0.694$ to $0.791$. Despite the performance difference in averaged accuracy, we observe a similar common-to-specialized trend on MCQ datasets, which matches our key observation that the performance of LLMs tends to downgrade as we go from common to specialized domains. }


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D8:} What is meant by an ``intermediate parent entity''? If an entity e is marked of type p, does this mean the benchmark only considers p? This seems to limit the questions too much. For example, A cat is a type of Mammal. And a Mammal is a type of Living Being. This implies that Cat is a Living Being too. Thus, being able to answer correctly that Cat is a mammal says nothing about the performance over inference tasks.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
Thanks for this discerning comment. An intermediate parent entity is its direct patent entity, and we have clarified this definition in Section~\ref{sec:question-design} in the revision. Suppose the root-to-leaf path is `Living Being'-`Mammal'-`Cat', and the possible ancestor-descendant pairs include `Living Being'-`Mammal', `Mammal'-`Cat', and `Living Being'-`Cat'. \textbf{Our main experiments} cover the former two pairs, which represent the fine-grained analysis of the root-to-leaf path structures. The scale of our main experiments in this case is $\mathcal{O}(n*m)$, where $n$ is the depth of the taxonomy and $m$ is the number of leaves. If we evaluate all the possible ancestor-descendant pairs in the taxonomies, the number of all ancestor/descendant combinations will be $\mathcal{O}(n^2*m)$, which is too large, especially when the tree is deep. Therefore, after careful consideration of the scale and effect of experiments, we mainly focus on a fine-grained analysis of the root-to-leaf path using the intermediate parent entity. 

In fact, we have covered the ancestor/descendant typing mentioned in your example \textbf{from the instance typing aspect} as shown in Section~\ref{sec:exp-instance}, where we examine the performance of LLMs on answering whether a leaf entity is a type of its parent, grandparent, parent of the grandparent, ..., root parent. In your example, we covered all the parents to the leaf entity `Cat': `Mammal'-`Cat', and `Living Being'-`Cat' in the instance typing experiment of the Biology taxonomy {\color{black}(indeed, when jointly considering the main experiment, where we covered `Mammal'-`Cat' and `Living Being'-`Mammal', all three possible ancestor-descendant pairs on the exemplar root-to-leaf path are evaluated)}. The overall trend presented from the instance typing experiments matches our main experiments on different taxonomies.

{\color{black} Moreover, to study the two-hop biology example you raised, we conducted an additional case study on the biology taxonomy. We aim to analyze whether the LLMs can answer the grandparent-child relation (g-c) correctly given that they can answer the grandparent-parent (g-p) and parent-child (p-c) relations correctly in the biology domain. Specifically, we randomly sampled 385 triplets (grandparent-parent-child) from the biology taxonomy following the sample size computation rule discussed in~\cite{Qualtrics}. We examined the performance of LLMs in answering the g-c under the condition that they correctly answered g-p and p-c. For ease of presentation, we treat the case where the model responds `I don't know' as the model wrongly answers the question. We present the experimental results in Table~\ref{tab:d8-case}, where the conditional accuracy measures the accuracy of the two-hop relation g-c under the prior condition that the LLMs correctly answer g-p and p-c. The overall accuracy is the accuracy of the two-hop relation g-c under all possible prior conditions. We notice that except for Llama-2-7B, all LLMs have over $90\%$ conditional accuracy, which means if the LLMs can answer the g-p and p-c relations correctly, it is highly likely that they can also accurately answer g-c. The reason why the conditional accuracy of Llama-2-7B is n/a is because the number of triplets where the model correctly answers both g-p and p-c is 0. As a result, we cannot measure its conditional accuracy. We further notice that the conditional accuracies of LLMs are higher than the overall accuracies of LLMs, indicating that when the LLMs cannot answer both g-p and p-c correctly, they can also not well capture the g-c relations. Therefore, although \textit{being able to answer correctly that Cat is a Mammal says nothing about the performance of answering Cat is a Living Being}, knowing the performance of answering Cat is a Mammal and Mammal is a Living Being gives a rough implication of the performance of answering Cat is a Living Being. We believe that by analyzing the LLMs with the fine-grained direct parent relationship, we can have a rough understanding of the LLMs' performance in handling the two-hop relationships you mentioned. Therefore, we focus on the fine-grained analysis of the root-to-leaf path using the intermediate parent entity.}

\begin{table}[t!]
  \caption{Case Study for R3-D8}
  \label{tab:d8-case}
  \begin{tabular}{lcc}
    \Xhline{0.8pt}
    \textbf{LLMs} & \textbf{conditional accuracy} & \textbf{overall accuracy}\\
    \hline
    GPT-3.5 & 0.962 & 0.813\\
    GPT-4 & 0.956 & 0.712\\
    Claude-3 & 0.979 & 0.842\\
    Llama-2-7B & n/a & 0.034\\
    Llama-2-13B & 0.977 & 0.719\\
    Llama-2-70B & 0.942 & 0.719\\
    Llama-3-8B & 0.991 & 0.899\\
    Llama-3-70B & 0.962 & 0.917\\
    Flan-T5-3B & 0.951 & 0.782 \\
    Flan-T5-11B & 1.000 & 0.725 \\
    Falcon-7B & 0.942 & 0.769\\
    Falcon-40B & 1.000 & 0.080\\
    Vicuna-7B & 0.980 & 0.961\\
    Vicuna-13B & 0.977 & 0.891\\
    Vicuna-33B & 0.988 & 0.899\\
    Mistral & 0.941 & 0.735\\
    Mixtral & 0.965 & 0.881\\
    LLMs4OL & 0.973 & 0.831\\
    \Xhline{0.8pt}
  \end{tabular}
   % end of color
   % end of font
\end{table}


%{\color{black}In summary, although we do not cover all the possible ancestor-descendant combinations in consideration of the scale and effect of the experiments. Our main experiments cover the fine-grained root-to-leaf path analysis for each level of the taxonomies; while our instance typing experiments cover some of the ancestor-descendant combinations (all the parents on the root-to-leaf path to the corresponding leaf entity).}

\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D9:} Section 4.4: This section needs more info on exactly how few-shot prompting and CoT were done.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
Apologize for any confusion. In our revised paper, we have added Figure~\ref{fig:few-cot} as an example to clarify the descriptions of the few-shot and chain-of-thoughts settings.


\vspace*{2ex}
\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable,boxsep=-1mm]
\textbf{D10:} Some of the LLMs mentioned in Limitations are indeed as old as 2017. It is unclear why they have not been included in the study. It is also unclear why LLM4OL was not compared within the experiments. Even though it works with limited domains, being the only nearest system, its results are important for the study.
\end{tcolorbox} 

\vspace*{-2ex}
\stitle{[A]}
First, we clarify that all the LLMs mentioned in Limitations are indeed later than 2023. Specifically, Falcon-180B~\cite{almazrouei2023falcon}, Claude-v2.1~\cite{Claude-v2.1-documentation}, and Mistral~\cite{jiang2023mistral} were released in 2023, while the Mixtral~\cite{jiang2024mixtral} model was released in 2024. We agree that including more baselines can improve the quality of the manuscript. Therefore, we selected Claude-3-Opus~\cite{Claude-v3-documentation} (the updated version of the Claude-v2.1), Mistral~\cite{jiang2023mistral}, and Mixtral~\cite{jiang2024mixtral} in the revised manuscript. 

The reasons why we did not include Falcon-180B are: 

\bi
    \item The deployment of the Falcon-180B model requires more than 400GB of memory, which we were unable to experiment with due to hardware constraints. 
    \item The Falcon-180B model is shown to be outperformed by Claude-3, Mistral, and Mixtral models according to the LMSYS Chatbot Arena Leaderboard (\url{https://chat.lmsys.org/?leaderboard}). 
\ei

Therefore, including the other three models would be of greater benefit to the improvement of our manuscript. We also included new SOTA models Llama-3-8B and Llama-3-70B~\cite{llama3modelcard}, which were just released on 18th April 2024 (see {\bf M2}). 

Besides, we also included LLMs4OL~\cite{babaei2023llms4ol} in our experiments following your suggestions (see {\bf M2}). The original implementation of the LLMs4OL model is limited in general, geography, and medical domains. We adapted and fine-tuned the model to other taxonomy domains by preserving the official implementation details~\cite{llms4ol-code} suggested by LLMsOL as much as possible, such as the model hyperparameters and train-test ratio. Please check Sections~\ref{sec:llms}, and~\ref{sec:implementation-details} for more details. 

\begin{table*}[t!]
\footnotesize
%\renewcommand\arraystretch{1.2}
  \caption{Accuracy with different variants of question templates on Easy Datasets.}
  \label{tab:exp-main-easy-revision}
  \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\textbf{eBay}}&\multicolumn{1}{c|}{\textbf{Amazon}}&\multicolumn{1}{c|}{\textbf{Google}}&\multicolumn{1}{c|}{\textbf{Schema}}&\multicolumn{1}{c|}{\textbf{ACM-CCS}}&\multicolumn{1}{c|}{\textbf{GeoNames}}&\multicolumn{1}{c|}{\textbf{Glottolog}}&\multicolumn{1}{c|}{\textbf{ICD-10-CM}}&\multicolumn{1}{c|}{\textbf{OAE}}&\multicolumn{1}{c}{\textbf{NCBI}}\\
    \hline
    \multirow{4}{*}{GPT-3.5} & v1 &0.921&0.775&0.920&0.593&0.711&0.598&0.563&0.851&0.778&0.529
  \\
    & v2 & 0.919&0.762&0.918&0.639&0.678&0.602&0.539&0.843&0.723&0.501
 \\
    & v3 & 0.908&0.720&0.890&0.580&0.613&0.598&0.481&0.803&0.597&0.445
 \\
    & std & 0.006&0.023&0.014&0.025&0.041&0.002&0.034&0.021&0.076&0.035
\\
    \multirow{4}{*}{GPT-4} & v1 & 0.946&0.879&0.962&0.773&0.860&0.648&0.710&0.964&0.866&0.789
  \\
    & v2 & 0.946&0.880&0.962&0.755&0.864&0.663&0.698&0.960&0.889&0.803
 \\
    & v3 & 0.947&0.878&0.962&0.794&0.857&0.697&0.653&0.955&0.867&0.782
\\
    & std & 0.000&0.001&0.000&0.016&0.003&0.020&0.025&0.004&0.011&0.009
\\
\hline
    \multirow{4}{*}{Claude-3} & v1 &  0.932&0.758&0.910&0.331&0.784&0.679&0.256&0.953&0.869&0.486
 \\
    & v2 & 0.932&0.761&0.907&0.389&0.774&0.669&0.271&0.945&0.866&0.494
 \\
    & v3 & 0.919&0.736&0.889&0.406&0.757&0.681&0.250&0.931&0.815&0.504
\\
    & std &0.006&0.011&0.009&0.032&0.011&0.005&0.009&0.009&0.025&0.007
\\
    \hline
    \multirow{4}{*}{Llama-2-7B} & v1 & 0.196&0.053&0.090&0.000&0.032&0.006&0.001&0.115&0.004&0.000
 \\
    & v2 & 0.257&0.081&0.167&0.001&0.046&0.010&0.002&0.137&0.005&0.001
 \\
    & v3 & 0.201&0.072&0.147&0.001&0.035&0.010&0.001&0.126&0.005&0.000
\\
    & std & 0.028&0.012&0.033&0.000&0.006&0.002&0.000&0.009&0.000&0.000
\\
    \multirow{4}{*}{Llama-2-13B} & v1 & 0.926&0.798&0.886&0.727&0.789&0.543&0.149&0.815&0.714&0.411
 \\
    & v2 & 0.927&0.817&0.904&0.747&0.778&0.543&0.133&0.832&0.795&0.417
 \\
    & v3 & 0.929&0.827&0.922&0.778&0.747&0.541&0.124&0.806&0.764&0.359
\\
    & std & 0.001&0.012&0.015&0.021&0.018&0.001&0.010&0.011&0.033&0.026
\\
    \multirow{4}{*}{Llama-2-70B} & v1 & 0.931&0.865&0.945&0.616&0.817&0.553&0.292&0.884&0.761&0.536
\\
    & v2 & 0.932&0.867&0.947&0.638&0.831&0.553&0.266&0.873&0.800&0.507
 \\
    & v3 & 0.934&0.862&0.944&0.643&0.819&0.573&0.215&0.851&0.741&0.425
\\
    & std & 0.001&0.002&0.001&0.012&0.006&0.009&0.032&0.014&0.024&0.047

\\
    \hline
    \multirow{4}{*}{Llama-3-8B} & v1 & 0.931&0.871&0.940&0.819&0.829&0.663&0.665&0.915&0.893&0.785
 \\
    & v2 & 0.937&0.873&0.942&0.821&0.822&0.681&0.668&0.917&0.905&0.784
 \\
    & v3 & 0.931&0.874&0.934&0.862&0.813&0.720&0.638&0.904&0.905&0.788
\\
    & std & 0.003&0.001&0.003&0.020&0.007&0.024&0.013&0.006&0.006&0.002


\\
    \multirow{4}{*}{Llama-3-70B} & v1 & 0.939&0.797&0.927&0.376&0.787&0.693&0.354&0.899&0.804&0.514
\\
    & v2 & 0.932&0.797&0.928&0.427&0.795&0.732&0.346&0.895&0.797&0.539
 \\
    & v3 & 0.931&0.747&0.894&0.426&0.759&0.750&0.281&0.871&0.670&0.506
\\
    & std & 0.004&0.024&0.016&0.024&0.015&0.024&0.033&0.012&0.062&0.014
\\
\hline
    \multirow{4}{*}{Flan-T5-3B} & v1 & 0.926&0.826&0.934&0.751&0.732&0.539&0.588&0.811&0.851&0.605
 \\
    & v2 & 0.934&0.837&0.941&0.793&0.752&0.575&0.598&0.819&0.867&0.614
 \\
    & v3 & 0.927&0.826&0.934&0.796&0.754&0.638&0.600&0.819&0.883&0.625
\\
    & std & 0.004&0.005&0.003&0.021&0.010&0.041&0.005&0.004&0.013&0.008
\\
    \multirow{4}{*}{Flan-T5-11B} & v1 & 0.944&0.834&0.944&0.804&0.737&0.520&0.595&0.871&0.875&0.643
 \\
    & v2 & 0.944&0.822&0.940&0.815&0.734&0.530&0.595&0.873&0.880&0.637
 \\
    & v3 & 0.936&0.821&0.940&0.808&0.742&0.526&0.594&0.863&0.884&0.630
\\
    & std & 0.004&0.006&0.002&0.005&0.003&0.004&0.000&0.004&0.004&0.005
\\
    \hline
    \multirow{4}{*}{Falcon-7B} & v1 & 0.607&0.553&0.574&0.504&0.577&0.533&0.504&0.677&0.495&0.618
\\
    & v2 &  0.667&0.571&0.613&0.513&0.604&0.535&0.505&0.693&0.498&0.609
\\
    & v3 & 0.675&0.566&0.610&0.512&0.602&0.561&0.503&0.689&0.510&0.574
\\
    & std & 0.030&0.008&0.018&0.004&0.012&0.013&0.001&0.007&0.006&0.019
\\
    \multirow{4}{*}{Falcon-40B} & v1 & 0.434&0.255&0.357&0.013&0.042&0.106&0.021&0.449&0.005&0.012
\\
    & v2 & 0.441&0.275&0.385&0.008&0.034&0.126&0.021&0.477&0.011&0.014
 \\
    & v3 & 0.393&0.236&0.358&0.004&0.039&0.128&0.014&0.422&0.014&0.014
\\
    & std & 0.021&0.016&0.013&0.004&0.003&0.010&0.003&0.022&0.004&0.001
\\
        \hline
    \multirow{4}{*}{Vicuna-7B} & v1 & 0.919&0.814&0.915&0.723&0.748&0.705&0.671&0.877&0.878&0.676
\\
    & v2 & 0.916&0.809&0.918&0.695&0.748&0.697&0.678&0.880&0.887&0.675
\\
    & v3 & 0.911&0.798&0.910&0.782&0.715&0.693&0.684&0.869&0.874&0.648
\\
    & std & 0.003&0.007&0.003&0.036&0.016&0.005&0.005&0.005&0.005&0.013
\\
    \multirow{4}{*}{Vicuna-13B} & v1 & 0.812&0.708&0.741&0.580&0.575&0.492&0.297&0.668&0.409&0.347
 \\
    & v2 & 0.814&0.727&0.753&0.569&0.575&0.500&0.302&0.680&0.466&0.361
 \\
    & v3 & 0.822&0.711&0.748&0.599&0.575&0.490&0.256&0.669&0.458&0.353
\\
    & std & 0.004&0.008&0.005&0.012&0.000&0.004&0.021&0.005&0.025&0.006

\\
    \multirow{4}{*}{Vicuna-33B} & v1 & 0.871&0.839&0.857&0.792&0.737&0.728&0.536&0.887&0.887&0.601
\\
    & v2 & 0.876&0.837&0.853&0.833&0.730&0.730&0.450&0.878&0.892&0.591
 \\
    & v3 & 0.906&0.839&0.892&0.840&0.767&0.717&0.430&0.858&0.882&0.607
\\
    & std & 0.015&0.001&0.018&0.021&0.016&0.006&0.046&0.012&0.004&0.007
\\
    \hline
    \multirow{4}{*}{Mistral} & v1 & 0.571&0.460&0.509&0.211&0.428&0.240&0.146&0.467&0.405&0.176
\\
    & v2 & 0.559&0.450&0.503&0.226&0.416&0.246&0.132&0.463&0.405&0.179
 \\
    & v3 & 0.566&0.429&0.504&0.204&0.409&0.299&0.105&0.462&0.401&0.152
\\
    & std & 0.005&0.013&0.003&0.009&0.008&0.027&0.017&0.002&0.002&0.012

\\
    \multirow{4}{*}{Mixtral} & v1 & 0.898&0.829&0.894&0.745&0.656&0.604&0.369&0.873&0.809&0.451
\\
    & v2 & 0.894&0.823&0.868&0.736&0.711&0.671&0.477&0.888&0.852&0.533
 \\
    & v3 & 0.883&0.820&0.863&0.751&0.728&0.622&0.476&0.882&0.864&0.547
\\
    & std & 0.006&0.004&0.014&0.006&0.031&0.028&0.051&0.006&0.024&0.042

\\
    \hline
    \multirow{4}{*}{LLMs4OL} & v1 & 0.929&0.890&0.908&0.932&0.844&0.677&0.739&0.935&0.933&0.748
\\
    & v2 &  0.927&0.890&0.906&0.932&0.848&0.683&0.735&0.936&0.932&0.750
\\
    & v3 & 0.927&0.895&0.904&0.932&0.848&0.693&0.736&0.933&0.934&0.748
\\
    & std & 0.001&0.002&0.002&0.000&0.002&0.007&0.002&0.001&0.001&0.001



\\
    \hline
  \end{tabular}
\end{table*}    


\begin{table*}[t!]
\footnotesize
%\renewcommand\arraystretch{1.2}
  \caption{Accuracy with different variants of question templates on Hard Datasets.}
  \label{tab:exp-main-hard-revision}
  \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\textbf{eBay}}&\multicolumn{1}{c|}{\textbf{Amazon}}&\multicolumn{1}{c|}{\textbf{Google}}&\multicolumn{1}{c|}{\textbf{Schema}}&\multicolumn{1}{c|}{\textbf{ACM-CCS}}&\multicolumn{1}{c|}{\textbf{GeoNames}}&\multicolumn{1}{c|}{\textbf{Glottolog}}&\multicolumn{1}{c|}{\textbf{ICD-10-CM}}&\multicolumn{1}{c|}{\textbf{OAE}}&\multicolumn{1}{c}{\textbf{NCBI}}\\
    \hline
    \multirow{4}{*}{GPT-3.5} & v1 &0.891&0.724&0.814&0.591&0.617&0.598&0.510&0.838&0.767&0.495
  \\
    & v2 & 0.884&0.712&0.808&0.642&0.590&0.602&0.488&0.839&0.720&0.486
 \\
    & v3 & 0.876&0.684&0.791&0.596&0.549&0.598&0.435&0.791&0.628&0.443
 \\
    & std & 0.006&0.017&0.010&0.023&0.028&0.002&0.031&0.022&0.058&0.023
\\
    \multirow{4}{*}{GPT-4} & v1 & 0.921&0.806&0.857&0.734&0.708&0.652&0.626&0.917&0.822&0.653
  \\
    & v2 & 0.916&0.805&0.859&0.720&0.693&0.665&0.609&0.910&0.845&0.669
 \\
    & v3 & 0.916&0.804&0.851&0.744&0.681&0.699&0.565&0.908&0.822&0.644
\\
    & std & 0.002&0.001&0.003&0.010&0.011&0.020&0.026&0.004&0.011&0.010
\\
\hline
    \multirow{4}{*}{Claude-3} & v1 &  0.901&0.668&0.781&0.315&0.624&0.679&0.244&0.871&0.766&0.449
  \\
    & v2 & 0.891&0.660&0.771&0.364&0.626&0.667&0.259&0.866&0.761&0.457
 \\
    & v3 & 0.858&0.632&0.743&0.380&0.611&0.681&0.243&0.851&0.695&0.459
\\
    & std & 0.018&0.015&0.016&0.028&0.007&0.006&0.007&0.008&0.032&0.004
\\
    \hline
    \multirow{4}{*}{Llama-2-7B} & v1 & 0.201&0.052&0.092&0.000&0.032&0.006&0.001&0.114&0.004&0.000
 \\
    & v2 & 0.264&0.079&0.170&0.001&0.047&0.010&0.002&0.137&0.005&0.001
 \\
    & v3 & 0.203&0.073&0.151&0.001&0.035&0.010&0.001&0.126&0.005&0.000
\\
    & std & 0.029&0.012&0.033&0.000&0.006&0.002&0.000&0.009&0.000&0.000
\\
    \multirow{4}{*}{Llama-2-13B} & v1 & 0.898&0.766&0.822&0.712&0.658&0.543&0.192&0.811&0.757&0.457
 \\
    & v2 & 0.898&0.780&0.829&0.730&0.639&0.543&0.182&0.810&0.809&0.457
 \\
    & v3 & 0.891&0.775&0.821&0.755&0.620&0.541&0.165&0.802&0.779&0.390
\\
    & std & 0.003&0.006&0.004&0.018&0.016&0.001&0.011&0.004&0.021&0.032
\\
    \multirow{4}{*}{Llama-2-70B} & v1 & 0.899&0.806&0.836&0.616&0.687&0.553&0.305&0.826&0.747&0.535
 \\
    & v2 & 0.899&0.804&0.822&0.638&0.690&0.553&0.287&0.818&0.782&0.510
 \\
    & v3 & 0.894&0.798&0.810&0.644&0.661&0.573&0.234&0.804&0.726&0.438
\\
    & std & 0.002&0.003&0.011&0.012&0.013&0.009&0.030&0.009&0.023&0.041
\\
    \hline
    \multirow{4}{*}{Llama-3-8B} & v1 & 0.880&0.789&0.774&0.788&0.664&0.663&0.608&0.878&0.851&0.691
\\
    & v2 & 0.886&0.793&0.780&0.787&0.652&0.681&0.609&0.876&0.867&0.688
 \\
    & v3 & 0.870&0.781&0.767&0.812&0.637&0.720&0.577&0.867&0.857&0.678
\\
    & std & 0.007&0.005&0.005&0.012&0.011&0.024&0.015&0.005&0.007&0.006
\\
    \multirow{4}{*}{Llama-3-70B} & v1 & 0.904&0.770&0.824&0.419&0.705&0.693&0.388&0.881&0.800&0.551
\\
    & v2 & 0.904&0.767&0.816&0.468&0.702&0.732&0.378&0.880&0.790&0.558
\\
    & v3 & 0.896&0.741&0.797&0.470&0.684&0.750&0.305&0.866&0.718&0.533
\\
    & std & 0.004&0.013&0.011&0.024&0.009&0.024&0.037&0.007&0.037&0.011
\\
    \hline
    \multirow{4}{*}{Flan-T5-3B} & v1 & 0.899&0.781&0.835&0.743&0.672&0.539&0.584&0.767&0.838&0.593
 \\
    & v2 & 0.906&0.783&0.829&0.768&0.683&0.575&0.593&0.767&0.848&0.600
 \\
    & v3 & 0.901&0.775&0.825&0.769&0.679&0.638&0.591&0.764&0.863&0.610
\\
    & std & 0.003&0.003&0.004&0.012&0.005&0.041&0.004&0.001&0.010&0.007
\\
    \multirow{4}{*}{Flan-T5-11B} & v1 & 0.919&0.793&0.864&0.786&0.698&0.520&0.589&0.842&0.856&0.633
 \\
    & v2 & 0.917&0.781&0.861&0.795&0.694&0.530&0.588&0.841&0.859&0.626
 \\
    & v3 & 0.908&0.782&0.855&0.789&0.696&0.526&0.586&0.830&0.860&0.620
\\
    & std & 0.005&0.005&0.004&0.004&0.002&0.004&0.001&0.005&0.002&0.005
\\
    \hline
    \multirow{4}{*}{Falcon-7B} & v1 & 0.597&0.547&0.556&0.501&0.550&0.537&0.503&0.636&0.497&0.587
 \\
    & v2 &  0.653&0.554&0.583&0.515&0.560&0.537&0.504&0.648&0.499&0.575
\\
    & v3 & 0.655&0.552&0.587&0.511&0.561&0.551&0.503&0.646&0.504&0.548
\\
    & std & 0.027&0.003&0.014&0.006&0.005&0.007&0.000&0.005&0.003&0.016
\\
    \multirow{4}{*}{Falcon-40B} & v1 & 0.434&0.253&0.348&0.013&0.043&0.108&0.021&0.454&0.007&0.013
 \\
    & v2 & 0.434&0.270&0.374&0.009&0.035&0.132&0.022&0.474&0.011&0.014
 \\
    & v3 & 0.393&0.237&0.359&0.006&0.039&0.132&0.015&0.442&0.014&0.014
\\
    & std & 0.019&0.013&0.011&0.003&0.003&0.011&0.003&0.013&0.003&0.000
\\
        \hline
    \multirow{4}{*}{Vicuna-7B} & v1 & 0.827&0.725&0.728&0.699&0.599&0.705&0.637&0.757&0.813&0.609
  \\
    & v2 & 0.818&0.733&0.737&0.681&0.601&0.697&0.635&0.761&0.814&0.603
 \\
    & v3 & 0.815&0.716&0.731&0.753&0.582&0.693&0.641&0.756&0.788&0.588
\\
    & std & 0.005&0.007&0.004&0.031&0.009&0.005&0.002&0.002&0.012&0.009
\\
    \multirow{4}{*}{Vicuna-13B} & v1 & 0.690&0.625&0.601&0.581&0.527&0.492&0.301&0.666&0.424&0.350
 \\
    & v2 & 0.682&0.620&0.596&0.576&0.527&0.500&0.304&0.676&0.480&0.361
\\
    & v3 & 0.688&0.619&0.602&0.599&0.526&0.490&0.259&0.667&0.471&0.354
\\
    & std & 0.003&0.003&0.003&0.010&0.000&0.004&0.021&0.004&0.025&0.005
\\
    \multirow{4}{*}{Vicuna-33B} & v1 & 0.759&0.713&0.682&0.728&0.591&0.728&0.496&0.772&0.820&0.522
  \\
    & v2 & 0.761&0.715&0.673&0.745&0.592&0.730&0.417&0.763&0.820&0.515
 \\
    & v3 & 0.802&0.730&0.713&0.780&0.609&0.717&0.405&0.763&0.802&0.543
\\
    & std & 0.020&0.008&0.017&0.022&0.008&0.006&0.040&0.004&0.008&0.012
\\
    \hline
    \multirow{4}{*}{Mistral} & v1 & 0.583&0.474&0.532&0.214&0.433&0.240&0.146&0.478&0.405&0.176
  \\
    & v2 & 0.583&0.464&0.521&0.227&0.421&0.246&0.132&0.475&0.405&0.179
 \\
    & v3 & 0.561&0.435&0.510&0.206&0.414&0.299&0.105&0.474&0.402&0.152
\\
    & std & 0.010&0.017&0.009&0.009&0.008&0.027&0.017&0.002&0.001&0.012
\\
    \multirow{4}{*}{Mixtral} & v1 & 0.805&0.739&0.738&0.707&0.618&0.604&0.394&0.840&0.789&0.482
 \\
    & v2 & 0.784&0.724&0.720&0.700&0.644&0.671&0.506&0.847&0.819&0.548
 \\
    & v3 & 0.771&0.719&0.704&0.697&0.644&0.622&0.508&0.839&0.832&0.563
\\
    & std & 0.014&0.008&0.014&0.004&0.012&0.028&0.053&0.004&0.018&0.035
\\
    \hline
    \multirow{4}{*}{LLMs4OL} & v1 & 0.904&0.849&0.860&0.912&0.753&0.677&0.711&0.891&0.906&0.725
 \\
    & v2 &  0.899&0.849&0.858&0.911&0.756&0.683&0.710&0.890&0.906&0.726
\\
    & v3 & 0.901&0.850&0.858&0.910&0.751&0.693&0.712&0.888&0.909&0.724
\\
    & std & 0.002&0.000&0.001&0.001&0.002&0.007&0.001&0.001&0.001&0.001\\
    \hline
  \end{tabular}
\end{table*}    

 
\begin{table*}[t!]
\footnotesize
%\renewcommand\arraystretch{1.2}
  \caption{Accuracy with different variants of question templates on MCQ Datasets.}
  \label{tab:exp-main-mcq-revision}
  \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multicolumn{1}{c|}{}&\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{\textbf{eBay}}&\multicolumn{1}{c|}{\textbf{Amazon}}&\multicolumn{1}{c|}{\textbf{Google}}&\multicolumn{1}{c|}{\textbf{Schema}}&\multicolumn{1}{c|}{\textbf{ACM-CCS}}&\multicolumn{1}{c|}{\textbf{GeoNames}}&\multicolumn{1}{c|}{\textbf{Glottolog}}&\multicolumn{1}{c|}{\textbf{ICD-10-CM}}&\multicolumn{1}{c|}{\textbf{OAE}}&\multicolumn{1}{c}{\textbf{NCBI}}\\
    \hline
    \multirow{4}{*}{GPT-3.5} & v1 &0.931&0.782&0.894&0.842&0.709&0.504&0.534&0.915&0.824&0.531
 \\
    & v2 & 0.941&0.775&0.891&0.826&0.702&0.545&0.500&0.884&0.817&0.495
\\
    & v3 & 0.921&0.744&0.885&0.802&0.660&0.435&0.484&0.899&0.775&0.475
\\
    & std & 0.008&0.017&0.004&0.016&0.022&0.045&0.021&0.013&0.022&0.023


\\
    \multirow{4}{*}{GPT-4} & v1 & 0.947&0.849&0.932&0.907&0.790&0.695&0.683&0.964&0.900&0.701
   \\
    & v2 & 0.954&0.845&0.930&0.911&0.768&0.687&0.687&0.964&0.901&0.701
 \\
    & v3 & 0.950&0.840&0.931&0.911&0.765&0.691&0.684&0.964&0.896&0.690
\\
    & std & 0.003&0.004&0.001&0.002&0.011&0.003&0.002&0.000&0.002&0.005
\\
\hline
    \multirow{4}{*}{Claude-3} & v1 &  0.947&0.830&0.922&0.894&0.741&0.638&0.497&0.962&0.885&0.577
 \\
    & v2 & 0.937&0.824&0.918&0.887&0.743&0.646&0.483&0.962&0.884&0.549
 \\
    & v3 & 0.941&0.815&0.919&0.890&0.726&0.630&0.501&0.955&0.876&0.586
\\
    & std & 0.004&0.006&0.002&0.003&0.008&0.007&0.008&0.003&0.004&0.016

\\
    \hline
    \multirow{4}{*}{Llama-2-7B} & v1 & 0.488&0.399&0.393&0.304&0.259&0.305&0.313&0.406&0.283&0.271
\\
    & v2 & 0.465&0.398&0.383&0.290&0.265&0.305&0.240&0.363&0.254&0.264
 \\
    & v3 & 0.472&0.390&0.393&0.336&0.279&0.305&0.321&0.449&0.323&0.289
\\
    & std & 0.010&0.004&0.005&0.019&0.008&0.000&0.036&0.035&0.028&0.011


\\
    \multirow{4}{*}{Llama-2-13B} & v1 & 0.680&0.551&0.547&0.448&0.450&0.313&0.305&0.695&0.429&0.368
\\
    & v2 & 0.644&0.528&0.513&0.432&0.429&0.309&0.277&0.658&0.383&0.349
 \\
    & v3 & 0.630&0.520&0.511&0.402&0.436&0.317&0.285&0.636&0.384&0.359
\\
    & std & 0.021&0.013&0.017&0.019&0.009&0.003&0.012&0.024&0.021&0.008


\\
    \multirow{4}{*}{Llama-2-70B} & v1 & 0.881&0.704&0.794&0.604&0.556&0.350&0.352&0.776&0.613&0.359
\\
    & v2 & 0.894&0.700&0.789&0.604&0.536&0.329&0.340&0.765&0.618&0.358
 \\
    & v3 & 0.868&0.689&0.778&0.550&0.540&0.317&0.326&0.756&0.605&0.339
\\
    & std & 0.011&0.006&0.007&0.025&0.009&0.014&0.011&0.008&0.005&0.009



\\
\hline
    \multirow{4}{*}{Llama-3-8B} & v1 & 0.865&0.725&0.817&0.689&0.610&0.431&0.449&0.896&0.813&0.449
\\
    & v2 & 0.871&0.726&0.819&0.678&0.611&0.431&0.438&0.891&0.810&0.457
 \\
    & v3 & 0.868&0.703&0.817&0.664&0.603&0.386&0.419&0.884&0.795&0.437
\\
    & std & 0.002&0.011&0.001&0.010&0.004&0.021&0.012&0.005&0.008&0.008
\\
    \multirow{4}{*}{Llama-3-70B} & v1 & 0.941&0.790&0.898&0.805&0.729&0.598&0.634&0.956&0.905&0.650


 \\
    & v2 & 0.941&0.784&0.900&0.805&0.713&0.569&0.628&0.951&0.901&0.642
 \\
    & v3 & 0.941&0.775&0.899&0.801&0.716&0.585&0.636&0.949&0.898&0.654
\\
    & std & 
0.000&0.006&0.001&0.002&0.007&0.012&0.003&0.003&0.003&0.005

\\
    \hline
    \multirow{4}{*}{Flan-T5-3B} & v1 & 0.898&0.756&0.878&0.799&0.664&0.455&0.506&0.836&0.777&0.524
 \\
    & v2 & 0.891&0.753&0.877&0.795&0.656&0.447&0.495&0.826&0.733&0.509
 \\
    & v3 & 0.891&0.751&0.876&0.796&0.651&0.423&0.513&0.833&0.731&0.496
\\
    & std & 0.003&0.002&0.001&0.002&0.005&0.014&0.007&0.004&0.021&0.011
\\
    \multirow{4}{*}{Flan-T5-11B} & v1 & 0.904&0.805&0.902&0.841&0.696&0.634&0.583&0.877&0.817&0.550
\\
    & v2 & 0.901&0.797&0.900&0.840&0.694&0.622&0.574&0.867&0.801&0.541
 \\
    & v3 & 0.904&0.793&0.887&0.831&0.676&0.589&0.582&0.840&0.791&0.546
\\
    & std & 0.001&0.005&0.007&0.004&0.009&0.019&0.004&0.016&0.011&0.004


\\
    \hline
    \multirow{4}{*}{Falcon-7B} & v1 & 0.261&0.259&0.275&0.233&0.240&0.256&0.260&0.254&0.262&0.255
\\
    & v2 &  0.261&0.261&0.273&0.244&0.249&0.268&0.254&0.252&0.242&0.271
\\
    & v3 & 0.257&0.283&0.291&0.240&0.236&0.248&0.251&0.231&0.254&0.257
\\
    & std & 0.002&0.011&0.008&0.005&0.005&0.008&0.004&0.010&0.008&0.007


 \\
    \multirow{4}{*}{Falcon-40B} & v1 & 0.578&0.465&0.525&0.368&0.389&0.305&0.036&0.711&0.168&0.117
\\
    & v2 & 0.535&0.424&0.473&0.296&0.379&0.252&0.029&0.688&0.143&0.104
\\
    & v3 & 0.521&0.415&0.466&0.310&0.363&0.260&0.029&0.685&0.131&0.111
\\
    & std & 0.024&0.022&0.026&0.031&0.011&0.023&0.003&0.012&0.015&0.005



\\
        \hline
    \multirow{4}{*}{Vicuna-7B} & v1 & 0.617&0.493&0.527&0.425&0.384&0.313&0.409&0.528&0.473&0.392
\\
    & v2 & 0.647&0.556&0.572&0.421&0.394&0.325&0.414&0.542&0.462&0.398
 \\
    & v3 & 0.640&0.529&0.530&0.455&0.393&0.321&0.381&0.524&0.420&0.423
\\
    & std & 0.013&0.026&0.021&0.015&0.004&0.005&0.015&0.008&0.023&0.013
\\
    \multirow{4}{*}{Vicuna-13B} & v1 & 0.838&0.636&0.747&0.523&0.543&0.317&0.205&0.833&0.691&0.362
 \\
    & v2 & 0.845&0.639&0.740&0.554&0.519&0.289&0.187&0.818&0.647&0.344
 \\
    & v3 & 0.815&0.618&0.702&0.464&0.501&0.240&0.187&0.814&0.643&0.341
\\
    & std & 0.013&0.009&0.020&0.037&0.017&0.032&0.008&0.008&0.022&0.009


\\
    \multirow{4}{*}{Vicuna-33B} & v1 & 0.327&0.307&0.338&0.266&0.261&0.264&0.253&0.401&0.285&0.252
\\
    & v2 & 0.323&0.326&0.308&0.283&0.263&0.280&0.281&0.398&0.285&0.282
 \\
    & v3 & 0.343&0.313&0.339&0.276&0.274&0.280&0.258&0.412&0.310&0.250
\\
    & std & 0.009&0.008&0.014&0.007&0.006&0.008&0.012&0.006&0.012&0.015


\\
    \hline
    \multirow{4}{*}{Mistral} & v1 & 0.828&0.666&0.713&0.692&0.582&0.415&0.436&0.765&0.768&0.519
 \\
    & v2 & 0.828&0.665&0.707&0.688&0.568&0.407&0.417&0.767&0.761&0.522
 \\
    & v3 & 0.842&0.664&0.727&0.660&0.569&0.390&0.435&0.769&0.772&0.497
\\
    & std & 0.007&0.001&0.008&0.014&0.006&0.010&0.009&0.002&0.005&0.011


\\
    \multirow{4}{*}{Mixtral} & v1 & 0.924&0.768&0.876&0.775&0.707&0.537&0.611&0.923&0.797&0.634
 \\
    & v2 & 0.921&0.762&0.867&0.782&0.698&0.553&0.613&0.915&0.776&0.616
 \\
    & v3 & 0.921&0.762&0.871&0.784&0.709&0.533&0.609&0.918&0.778&0.626
\\
    & std & 0.001&0.003&0.004&0.004&0.005&0.009&0.002&0.003&0.009&0.007


\\
    \hline
    \multirow{4}{*}{LLMs4OL} & v1 & 0.954&0.851&0.924&0.921&0.796&0.683&0.660&0.921&0.941&0.650
 \\
    & v2 &  0.947&0.852&0.924&0.915&0.798&0.679&0.657&0.919&0.941&0.650
\\
    & v3 & 0.954&0.851&0.927&0.915&0.796&0.679&0.656&0.921&0.942&0.650
\\
    & std & 0.003&0.000&0.001&0.003&0.001&0.002&0.002&0.001&0.000&0.000

\\
    \hline
  \end{tabular}
\end{table*}    

%The intermediate parent entity is the lowest-level parent entity. For example, if we have a chain of entities that Cat is a type of Mammal and Mammal is a type of Living Being ($\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$), then the intermediate parent of Cat is Mammal. We have clarified the definition of the intermediate parent in \textbf{Question Generation} part of Section~\ref{sec:question-design} of our revised manuscript to make the concept clear. The reason why we focus on the intermediate parent when designing the T/F question templates is that the goal of this paper is to explore how well the LLMs can internalize the taxonomy structure. To achieve such a goal, we need to examine the performance of LLMs in answering ``Is Cat a type of Mammal'' and ``Is Mammal a type of Living Being'', so that we can evaluate the performance of LLMs in internalizing the complete chain structure ($\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$) in the taxonomy. If we evaluate the performance of LLMs in answering ``Is Cat a type of Living Being'', then we only know about the performance of LLMs in internalizing the structure $\text{Cat} \rightarrow \text{Living Being}$, the finer-grained structure of $\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$ remains unexplored. Therefore, to achieve a fine-grained analysis of the LLMs' ability to internalize taxonomy structures, we generate the questions based on the intermediate parent entity. 

%As for the Cat to Living Being inference, we think it is covered by the Instance Typing experiment as shown in Section~\ref{sec:exp-instance}, where we examine the performance of LLMs on answering whether a leaf entity is a type of its parent, grandparent, parent of the grandparent, ..., root parent: which indeed covers Cat to Living Being (the instance typing for entity to its grandparent on the biology NCBI taxonomy). The overall trend presented from the instance typing experiments matches with our main experiments on different taxonomies, which means on common taxonomies, the performance of LLMs is good enough to replace the traditional taxonomy structures, while on specialized taxonomies, the performance of LLMs is less stable and satisfactory.

%\hrulefill

%\begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable]
%	\textbf{R3-V1:} Further clarifications with respect to some claims/aspects. (D2, D4, D5, D6, D8, D9)

 %   \textbf{R3-W3:} Some of the details are skipped. Please refer to detailed feedback.
	
 %   \textbf{R3-D2:} Section 1: the definition of ``common'' vs ``specialized'' is only vaguely explained. For example, one may argue that ``Home \& Garden'' is indeed a specialized domain as compared to ``People''. How about using more general-purpose taxonomy as those of Wikidata or Schema.org (used by YAGO for e.g.)?

%    \textbf{R3-D4:} Section 2.1: The Amazon Product Category was crawled to collect it from BrowseNodes. What is the percentage coverage in this case w.r.t. the original catalog? The site mentions having only popular categories, thus, they could bias the end results.

%    \textbf{R3-D5:} Table 1: It is unclear how the number of entities is correlated with the specialization of the taxonomy. In general, the features chosen (levels, trees, etc.) to represent the diversity of the taxonomies are not concretely justified. What is the number of questions per taxonomy?

 %   \textbf{R3-D6:} Section 2.2: ``We observed similar results when using slight paraphrasing of the templates, so will report results on these templates only.'': What is meant by ``slight'' paraphrasing? How similar were the results?

 %   \textbf{R3-D8:} What is meant by an ``intermediate parent entity''? If an entity e is marked of type p, does this mean the benchmark only considers p? This seems to limit the questions too much. For example, A cat is a type of Mammal. And a Mammal is a type of Living Being. This implies that Cat is a Living Being too. Thus, being able to answer correctly that Cat is a mammal says nothing about the performance over inference tasks.

   %  \textbf{R3-D9:} Section 4.4: This section needs more info on exactly how few-shot prompting and CoT were done.
    
	
	% \end{tcolorbox}	

%\textbf{Response to R3-V1, and R3-W3.} Thank you for your comments. We have modified our manuscript based on your valuable suggestions accordingly. 

% \textbf{Response to R3-D2.} Thank you for your insightful comments. We agree that the definitions for common and specialized taxonomies are vaguely explained. Indeed, there is no universal definition of whether a taxonomy is common or specialized. Providing a formal definition for common and specialized taxonomies is indeed out of the scope of our research goal. Our goal here is to provide a rough, relative rank of commonness of different taxonomies that matches the common sense of the public so that we can summarize and demonstrate the experimental results on different taxonomies in a better way. In our revised manuscript, for ease of demonstration and discussion, we treat taxonomies that cover common entities known and accessible to ordinary people as common taxonomies while referring to the taxonomies that are domain-specific and likely to be accessed by domain experts as specialized taxonomies. We then classify the ten taxonomies into these two types based on the average number of results returned by google.com by searching (exact match) the names of 100 randomly sampled concepts from each taxonomy. The number of results returned by searching the sampled concept names can roughly reflect the level of commonness to the public of the taxonomies: If there is a large amount of information regarding a certain taxonomy's content on the internet, then it is likely that this taxonomy contains common information that is accessible to ordinary people; correspondingly, if the information on a certain taxonomy's content is scarce on the internet, then it is likely to be a specialized taxonomy used by experts in a certain domain. Some previous studies also adopted a similar way to estimate the popularity of the content based on the Google search results~\cite{malagon2023measuring, genoe2021applying}.

% As for the example of Home \& Garden and People, we have to admit that common taxonomies will also contain relatively domain-specific knowledge. Therefore, in our revised manuscript we measure the popularity as the average number of results returned by google.com by searching (exact match) the names of 100 randomly sampled concepts from each taxonomy. In this way, we can compare the overall level of commonness between any two different taxonomies and get a rough ranking of the commonness of taxonomies from common to specialized for ease of demonstration and discussion. 

% We agree that including the general-purpose taxonomy can improve the coverage of the benchmark paper. We therefore followed your suggestions and included Schema.org into our benchmark. We appreciate your suggestions and hope that the explanation and the inclusion of general-purpose taxonomy resolve your concerns.

%\textbf{Response to R3-D4.} Thank you for your comments. We agree that it is important to ensure the data coverage of the collected taxonomy, therefore we investigated the coverage of the collected Amazon Product Category. We first noticed that the BrowseNodes website did not mention that it has only popular categories. The statement on the website (\url{https://www.browsenodes.com/}) is indeed ``\textit{These are the top most browse nodes in Amazon.com.}'', which means the categories shown on that page are the root level nodes and does not imply the popularity of the nodes. 

% As for the coverage of the collected taxonomy over the original taxonomy, since Amazon only discloses the root categories on its official website (\url{https://www.amazon.com/}), we compared the root categories of the collected taxonomy and the original taxonomy and found that our collected taxonomy covers 39 out of 55 of the latest root categories of Amazon.com, which is over $70\%$ coverage. Indeed the Amazon Product Category is updated along with the development of its business, and thus the changes to the categories happen. 

% The main reason why we cannot obtain the full, original Amazon product taxonomy is that the complete Amazon Product Category is not publicly available. A state-registered merchant account is needed for API access to the complete Amazon Product Category. Therefore, we resort to the BrowseNodes website, which is built by caching the API access to the Amazon Product Category (as discussed in its information page: \url{https://www.commercedna.com/}), and thus some of the marginal categories are not covered by collected taxonomy. We believe crawling the BrowseNodes version of the Amazon Product Category is the best effort we can make as researchers without API access to the complete Amazon Product Category currently. 

% We released the crawling code on the GitHub repository of our paper (\url{https://github.com/ysunbp/TaxoGlimpse/tree/main/LLM-taxonomy/shopping}) and would like to update the Amazon Product Category and the benchmark results on the crawled Amazon Product Category frequently on the GitHub repository so that the community can obtain the up-to-date cached Amazon Product Category and the corresponding results for their reference. 

% Besides, we think the collected taxonomy can provide useful insights for the LLMs' application in shopping domain taxonomy. In order to ensure the reliability of the findings in the shopping domain, we have Google Product Category~\cite{Google-shopping-tax} as a reference in our original manuscript. We also included a new complete shopping taxonomy named eBay Categories, which is used by another widely used shopping website eBay.com to strengthen the reliability of the observations in the shopping domain. Please refer to Section~\ref{sec:data-collection} for the details. We observe that the results of the three shopping taxonomies are consistent and do not influence our observations and insights. 

% \textbf{Response to R3-D5.} Thank you for your comments. Indeed the number of entities is not correlated with the specialization of the taxonomy. In Section~\ref{sec:data-collection} of the original manuscript, we stated that ``\textit{Apart from the popularity of taxonomies, we also considered the characteristics of different taxonomies. As shown in Table~\ref{tab:taxonomies}, the selected taxonomies have a range of cover of different numbers of entities (from 2K to 2M), number of levels (from 4 to 7), and number of tree roots (from 13 to 245), represent well the overall distribution of taxonomies in different application scenarios.}'', which means the taxonomies we chose for evaluation are not only diverse in popularity but also have diverse features such as number of entities, number of levels, and number of tree roots. As a result, from the morphological perspective, the selected taxonomies have diverse structures, which means they are representative candidates for our evaluation. The main reason why we presented levels, trees, etc in Table~\ref{tab:taxonomies} is that these features describe the basic information of the taxonomies well. By having these features, the audience can learn about the scale of the taxonomies (number of entities), the depth of the taxonomies (number of levels), the width of the taxonomies (number of trees), the rough shape of the taxonomies (number of nodes and classes in each level), which gives the audience rough ideas of the characteristics of the taxonomies. We have updated Section~\ref{sec:data-collection} to explain further the relationship between the diversity of features and the representative of the taxonomies and justify the selection of these features. Specifically, we modified the paragraph into: ``\textit{Apart from the popularity of taxonomies, we also considered the characteristics of different taxonomies. As shown in Table~\ref{tab:taxonomies}, the characteristics we selected give the audience the basic information about the scale of the taxonomies (number of entities), the depth of the taxonomies (number of levels), the width of the taxonomies (number of trees), the rough shape of the taxonomies (number of nodes and classes in each level). The selected taxonomies have a range of cover of different numbers of entities (from 500 to 2M), number of levels (from 2 to 7), and number of tree roots (from 3 to 245), representing well the diverse distribution of the morphology of taxonomies in different application domains and scenarios.}'' As for the number of questions per taxonomy, we admit that our original presentation of Table~\ref{tab:data-stat} is not clear enough, we therefore added a new row at the bottom of the table recording the total number of questions per taxonomy. Please check Table~\ref{tab:data-stat} in the revised manuscript for details.

\begin{comment}

\begin{table*}[t!]
\footnotesize
  \caption{Statistics of Datasets.}
  \label{tab:data-stat}
  \begin{tabular}{@{}ll|l|l|l|l|l|l|l|l|l|l}
\hline
     & & \textbf{Google} & \textbf{Amazon} & \textbf{ICD-10-CM} & \textbf{ACM-CCS} & \textbf{NCBI} & \textbf{Glottolog}& \textbf{eBay}& \textbf{OAE}& \textbf{Schema}& \textbf{GeoNames}\\
    \hline
    \multirow{3}{*}{Level 1-root} & Easy &   258     &   438     &    222       &   138      &  344    &    500 & 176  & 638 &  34    & 492 \\ 
    \cline{2-12}
    ~ & Hard &   258    &   438     &    222       &   138      &  344    &    500 & 176   & 638  & 34  & 492\\ 
    \cline{2-12}
    ~ & MCQ &  129 & 219 & 111 & 69 & 172 & 250 & 88 & 319 & 17 & 246 \\ 
    \hline
    \multirow{3}{*}{Level 2-1}                          & Easy &   600     &   700     &    550       &   450      &  440    &    564   &  430  & 700  & 276  &  n/a\\ \cline{2-12}
    ~ & Hard &   597     &   700     &    550       &   450      &  439    &    564   &  430  & 700  & 276 &  n/a\\ 
    \cline{2-12}
    ~ & MCQ & 300 &  350 & 275 & 225 & 220 & 282 & 215 & 350 & 138 & n/a\\ 
    \hline
    \multirow{3}{*}{Level 3-2}                          & Easy &   656     &   748     &    690       &   568      &  638    &     584  &  n/a  & 670 & 394 &  n/a\\ \cline{2-12}
    ~ & Hard &   653     &   748     &     690      &   567      &  636    &     584   &  n/a  & 670 & 394 &  n/a\\ 
    \cline{2-12}
    ~ & MCQ & 328 & 374 & 345 & 284 & 319 & 192 & n/a & 335 & 197 & n/a\\ 
    \hline
    \multirow{3}{*}{Level 4-3}                          & Easy &   636     &   758     &    n/a       &   386      &  742    &     600   &  n/a & 572  & 410 &  n/a\\ \cline{2-12}
    ~ & Hard &   626     &   758     &    n/a       &    370     &  741    &     600   &  n/a  & 572 & 410  &  n/a\\ 
    \cline{2-12}
    ~ & MCQ & 318 & 379 & n/a & 193 & 371 & 300 & n/a & 286 & 205 & n/a\\ 
    \hline
    \multirow{3}{*}{Level 5-4}                          & Easy &  n/a      &   n/a     &    n/a       &    n/a     &  766    &     732   &  n/a  &  n/a & 320 &  n/a\\ \cline{2-12}
    ~ & Hard &   n/a     &   n/a     &    n/a       &   n/a      &  766    &      732   &  n/a &  n/a  & 320 &  n/a\\ 
    \cline{2-12}
    ~ & MCQ &  n/a & n/a & n/a & n/a & 383 & 366 & n/a & n/a & 160 & n/a\\ 
    \hline
    \multirow{3}{*}{Level 6-5}                          & Easy & n/a       &  n/a      &    n/a       & n/a        &  770    &   n/a  &  n/a &  n/a   & n/a &  n/a\\ \cline{2-12}
    ~ & Hard & n/a       &  n/a      &    n/a       & n/a        &  770    &   n/a &  n/a &  n/a    & n/a &  n/a\\ 
    \cline{2-12}
    ~ & MCQ &  n/a & n/a & n/a & n/a & 385 & n/a & n/a & n/a & n/a & n/a \\ 
    \hline
    \multirow{3}{*}{Total}                          & Easy & 2150 & 2644 & 1462 & 1542 & 3700 & 2980 & 606 & 2580 & 1434 & 492\\ \cline{2-12}
    ~ & Hard & 2134 & 2644 & 1462 & 1525 & 3696 & 2980 & 606 & 2580 & 1434 & 492\\
    \cline{2-12}
    ~ & MCQ &  1075 & 1322 & 731 & 771 & 1850 & 1490 & 303 & 1290 & 717 & 246\\ 
\hline
  \end{tabular}
\end{table*}
    
\end{comment}







% \textbf{Response to R3-D8.} Thank you for your helpful comments. The intermediate parent entity is the lowest-level parent entity. For example, if we have a chain of entities that Cat is a type of Mammal and Mammal is a type of Living Being ($\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$), then the intermediate parent of Cat is Mammal. We have clarified the definition of the intermediate parent in \textbf{Question Generation} part of Section~\ref{sec:question-design} of our revised manuscript to make the concept clear. The reason why we focus on the intermediate parent when designing the T/F question templates is that the goal of this paper is to explore how well the LLMs can internalize the taxonomy structure. To achieve such a goal, we need to examine the performance of LLMs in answering ``Is Cat a type of Mammal'' and ``Is Mammal a type of Living Being'', so that we can evaluate the performance of LLMs in internalizing the complete chain structure ($\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$) in the taxonomy. If we evaluate the performance of LLMs in answering ``Is Cat a type of Living Being'', then we only know about the performance of LLMs in internalizing the structure $\text{Cat} \rightarrow \text{Living Being}$, the finer-grained structure of $\text{Cat} \rightarrow \text{Mammal} \rightarrow \text{Living Being}$ remains unexplored. Therefore, to achieve a fine-grained analysis of the LLMs' ability to internalize taxonomy structures, we generate the questions based on the intermediate parent entity. 

% As for the Cat to Living Being inference, we think it is covered by the Instance Typing experiment as shown in Section~\ref{sec:exp-instance}, where we examine the performance of LLMs on answering whether a leaf entity is a type of its parent, grandparent, parent of the grandparent, ..., root parent: which indeed covers Cat to Living Being (the instance typing for entity to its grandparent on the biology NCBI taxonomy). The overall trend presented from the instance typing experiments matches with our main experiments on different taxonomies, which means on common taxonomies, the performance of LLMs is good enough to replace the traditional taxonomy structures, while on specialized taxonomies, the performance of LLMs is less stable and satisfactory.

%\textbf{Response to R3-D9.} Thanks for your comments. We agree that the few-shot and chain-of-thoughts settings are not clearly explained. We added Figure~\ref{fig:few-cot} in our revised paper as an example of the few-shot and chain-of-thoughts settings for our experiments to make the descriptions clearer. 

\begin{comment}
\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{./img/few-shot-cot.pdf}
  \vspace{-2em}
  \caption{Few-shot and Chain-of-Thoughts examples.}
  \label{fig:few-cot}
\end{figure}
    
\end{comment}

% \begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable]
% %	\textbf{R3-V2:} The experiments need to include more domains of taxonomies. (D2, D3)

%  %       \textbf{R3-W1:} The construction of the benchmark is not very convincing.
        
%   %      \textbf{R3-D2:} Section 1: the definition of ``common'' vs ``specialized'' is only vaguely explained. For example, one may argue that ``Home \& Garden'' is indeed a specialized domain as compared to ``People''. How about using more general-purpose taxonomy as those of Wikidata or Schema.org (used by YAGO for e.g.)?
	
% 	\textbf{R3-D3:} Figure 2: There is a sudden fall in popularity after Amazon. There is a need for a better medium popularity dataset.
	
% 	\end{tcolorbox}	

% %\textbf{Response to R3-V2, R3-W1, and R3-D2.} We appreciate your helpful comments. We clarified the definition of common and specialized taxonomies, please refer to \textbf{Response to R3-D2} for details. We agree that including general-purpose taxonomy would be helpful. Therefore, we included Schema.org in our benchmark. 

% \textbf{Response to R3-D3.} Thank you for your comments. Indeed, our previous measure of popularity based on the number of search results by searching the taxonomy names may not accurately reflect the popularity of the content of the taxonomy. Firstly, some taxonomies do not have a formal or universal name, such as eBay categories~\cite{ebay} (do not have a formal name) and Google Product Category~\cite{Google-shopping-tax} (refer to as ``Google Product Category'' on its introductory page~\cite{Google-shopping-intro}, while as ``Google Product Taxonomy'' in its file name~\cite{Google-shopping-tax}). Besides, the names of the taxonomies themselves would bias the results. Many irrelevant results are returned when searching Amazon Product Category and Google Product Category since the words Amazon and Google are common words on the internet. As a result, the estimated popularity of the Amazon Product Category and the Google Product Category is significantly higher than the rest of the taxonomies. Your comment \textbf{R3-D2} (\textit{For example, one may argue that ``Home \& Garden'' is indeed a specialized domain as compared to ``People''.}) enlightens us to think deeper about the popularity measure of the taxonomies. The popularity of taxonomy should be measured by the popularity of the taxonomy concepts (such as ``Home \& Garden'' and ``People'') inside instead of that of taxonomy names. Therefore, we rectified our measure of popularity as follows: we randomly sampled 100 concepts from each taxonomy and then recorded the average number of results returned by Google.com by searching for the concept names. To avoid the irrelevant content returned, we adopted the exact match searching mode of the Google search engine. The updated popularity is shown in Figure~\ref{fig:popularity}. We observe that the sudden fall in popularity problem is resolved after we adopted the rectified measure of popularity. We have updated Figure~\ref{fig:popularity} and the corresponding description in the revised manuscript.
% %We searched and included Schema.org~\cite{guha2016schema}, eBay~\cite{ebay}, GeoNames~\cite{geonames}, and OAE~\cite{he2014oae} taxonomies in our benchmark, where Schema.org and eBay are better medium popularity taxonomies with higher popularity than that of ICD-10-CM. Compared with our original manuscript, the sudden fall in popularity after Amazon's Product Categories is reduced. The reason why the Google Product Category and Amazon's Product Categories have significantly higher popularity than the rest of the taxonomies is that these two taxonomies are widely used by e-commerce users and therefore the search engine is likely to obtain matched search results for these two taxonomies. Schema.org taxonomy is yet less likely to be accessed by layman internet users although it is a general domain taxonomy with a large number of users from the semantic web research community. Another shopping taxonomy eBay also has much smaller popularity compared with Amazon's Product Categories, since it is indeed a less popular e-commerce platform according to the statistics shown in~\cite{Amazon-shopping-stat}. {\color{black}Leave for Luna's response.}

\begin{comment}
\begin{figure}[t!]
  \centering
\includegraphics[width=1.0\linewidth]{./img/popularity.pdf}
\vspace{-1.5em}
  \caption{The Popularity of Different Taxonomies.}
  \label{fig:popularity}
\end{figure}
\end{comment}

%  \begin{tcolorbox}[notitle,boxrule=0pt,colback=gray!20,colframe=gray!20,breakable]
% %	\textbf{R3-V3:} Use of diverse benchmarks and baselines. (D7, D10)

%  %       \textbf{R3-W2:} The experiments are not thorough enough for an EA\&B paper.
        
% %        \textbf{R3-D7:} With LLMs, it is possible to have varied results on slight changes in the language structure and end task. Thus, simple True/False questions are in no way an exhaustive evaluation for LLMs over taxonomy-based end tasks. The authors cite [21] to suggest that True/False questions are better than MCQs for humans. This is, however, not conclusive for machine-based LLMs.
	
% 	\textbf{R3-D10:} Some of the LLMs mentioned in Limitations are indeed as old as 2017. It is unclear why they have not been included in the study. It is also unclear why LLM4OL was not compared within the experiments. Even though it works with limited domains, being the only nearest system, its results are important for the study.
	
% 	\end{tcolorbox}	

% \textbf{Response to R3-V3, and R3-D10.} Thank you for your comments. We first noticed that all the LLMs mentioned in Limitations are indeed later than 2023. Specifically, Falcon-180B~\cite{almazrouei2023falcon}, Claude-v2.1~\cite{Claude-v2.1-documentation}, and Mistral~\cite{jiang2023mistral} were released in 2023, while the Mixtral~\cite{jiang2024mixtral} model was released in 2024. We agree that including more baselines can improve the quality of the manuscript. Therefore, we selected Claude-3-Opus~\cite{Claude-v3-documentation} (the updated version of the Claude-v2.1), Mistral~\cite{jiang2023mistral}, and Mixtral~\cite{jiang2024mixtral} in the revised manuscript. The reasons why we did not include Falcon-180B are that 1) The deployment of the Falcon-180B model requires more than 400GB of memory, which we were unable to experiment with due to hardware constraints. 2) the Falcon-180B model is shown to be outperformed by the Claude-3, Mistral, and Mixtral models according to the LMSYS Chatbot Arena Leaderboard (\url{https://chat.lmsys.org/?leaderboard}). Therefore, we think including the other three models would be of greater benefit to the improvement of our manuscript. We also included new state-of-the-art models Llama-3-8B, and Llama-3-70B~\cite{llama3modelcard}, which were just released on 18th April 2024. Besides, we also included LLMs4OL~\cite{babaei2023llms4ol} in our experiments following your suggestions. The original implementation of the LLMs4OL model is limited in general, geography, and medical domains. We adapted and fine-tuned the model to other taxonomy domains by preserving the official implementation details~\cite{llms4ol-code} suggested by LLMsOL as much as possible. Please check Sections~\ref{sec:llms}, and~\ref{sec:implementation-details} for details. 



\begin{comment}
\begin{table*}[hbtp]
\setlength{\belowcaptionskip}{0.3cm}
  \caption{Summary of Changes.}
\centering
  \begin{tabular}{p{3cm}p{5cm}p{10cm}}
    \hline
    \textbf{Location} & \textbf{Comments} & \textbf{Changes}\\
    \hline
    Section 1 & R2-W1, R2-D2, R3-V2, R3-W1, and R3-D2 & We updated Figure~\ref{fig:example} to include added taxonomies.\\
    Section 2.1 & R3-D3 & We updated Figure 2 for the updated measure of popularity and included more taxonomies.\\
    Section 2.1 & R2-W1, R2-D2, R3-D5, R3-V2, R3-W1, and R3-D2 & Updated the statistics (Table 1) and the coverage of taxonomies, explained more on the diversity of the taxonomies. \\
    Section 2.2 & R3-V3, R3-W2, and R3-D7 & Added a new question type MCQ with detailed descriptions of its corresponding question templates and question generation methods.\\
    Section 2.2 & R3-D6 & Provided explanations on the similarity of the slight paraphrasing template variants.\\
    Section 2.2 & R3-D5 & Update the statistics of datasets generated in Table 4.\\
    Section 3.1 &R1-V1, R1-W1, R1-D2, R3-V3, and R3-D10 & Included more state-of-the-art LLMs.\\
    Section 4.1 & R3-D7, R2-W2, and R2-D1 & Added a paragraph discussing the effect of using different question types, which can also be considered as a new finding.\\
    Section 4.3 & R1-V2, R1-W2, R1-W3, R1-D4, R2-W2, and R2-D1& Added a discussion on the domain-specific instruction tuning.\\
    Section 4.4 & R3-D9 & Presented details of few-shot and CoT promptings.\\
    Section 4.4 & R2-V2, R2-W3, and R2-D3& Updated the visualization of the zero-shot, few-shot, and CoT results in Figure 4.\\
    Section 4.5 &R3-D8& Updated for added taxonomies. This section is related to the Comment R3-D8.\\ 
    Section 5.2 &R1-V1, and R1-W2& Added a section discussing the limitations of LLMs.\\
    Section 5.3 &R1-V3, and R1-D3& Added a case study on the integration of LLMs and taxonomy.\\
    Section 5.4 &R1-D4& Added the scalability analysis of LLMs.\\
    Overall & R2-W2, and R2-D1 & The revised manuscript has a wider coverage of LLMs and taxonomies, which strengthens the credibility of the insights. We expanded the findings on domain-specific instruction tuning. Besides, we discussed the limitations, provided a case study on the integration of LLM and taxonomy, and discussed the scalability of the LLMs. As a result, the insights and contributions of this paper are greatly enhanced.\\
    \hline
\end{tabular}
\label{tab:summary_change}
\end{table*}


\vspace*{2\baselineskip} 
	\textbf{\large Summary of Changes}
 \vspace*{1\baselineskip} 
 
 We summarize the changes in \autoref{tab:summary_change}. We hope the revisions have addressed all the concerns raised by the reviewers.

\end{comment}

\newpage

